Efficient Nonlinear Function Approximation in Analog Resistive Crossbars for Recurrent Neural Networks

Analog In-memory Computing (IMC) has demonstrated energy-efficient and low latency implementation of convolution and fully-connected layers in deep neural networks (DNN) by using physics for computing in parallel resistive memory arrays. However, recurrent neural networks (RNN) that are widely used for speech-recognition and natural language processing have tasted limited success with this approach. This can be attributed to the significant time and energy penalties incurred in implementing nonlinear activation functions that are abundant in such models. In this work, we experimentally demonstrate the implementation of a non-linear activation function integrated with a ramp analog-to-digital conversion (ADC) at the periphery of the memory to improve in-memory implementation of RNNs. Our approach uses an extra column of memristors to produce an appropriately pre-distorted ramp voltage such that the comparator output directly approximates the desired nonlinear function. We experimentally demonstrate programming different nonlinear functions using a memristive array and simulate its incorporation in RNNs to solve keyword spotting and language modelling tasks. Compared to other approaches, we demonstrate manifold increase in area-efficiency, energy-efficiency and throughput due to the in-memory, programmable ramp generator that removes digital processing overhead.

==> refbib <==
@incollection{paszke19pytorch,
title = {PyTorch: An Imperative Style, High-Performance Deep Learning Library},
author = {Paszke, Adam and Gross, Sam and Massa, Francisco and Lerer, Adam and Bradbury, James and Chanan, Gregory and Killeen, Trevor and Lin, Zeming and Gimelshein, Natalia and Antiga, Luca and Desmaison, Alban and Kopf, Andreas and Yang, Edward and DeVito, Zachary and Raison, Martin and Tejani, Alykhan and Chilamkurthy, Sasank and Steiner, Benoit and Fang, Lu and Bai, Junjie and Chintala, Soumith},
booktitle = {Advances in Neural Information Processing Systems 32},
pages = {8024--8035},
year = {2019},
publisher = {Curran Associates, Inc.},
url = {http://papers.neurips.cc/paper/9015-pytorch-an-imperative-style-high-performance-deep-learning-library.pdf}
}

@misc{SpikingJelly,
	title = {SpikingJelly},
	author = {Fang, Wei and Chen, Yanqi and Ding, Jianhao and Chen, Ding and Yu, Zhaofei and Zhou, Huihui and Timothée Masquelier and Tian, Yonghong and other contributors},
	year = {2020},
	howpublished = {\url{https://github.com/fangwei123456/spikingjelly}},
}

@ARTICLE{eshraghian2021training,
  author={Eshraghian, Jason K. and Ward, Max and Neftci, Emre O. and Wang, Xinxin and Lenz, Gregor and Dwivedi, Girish and Bennamoun, Mohammed and Jeong, Doo Seok and Lu, Wei D.},
  journal={Proceedings of the IEEE}, 
  title={Training Spiking Neural Networks Using Lessons From Deep Learning}, 
  year={2023},
  volume={111},
  number={9},
  pages={1016-1054},
  doi={10.1109/JPROC.2023.3308088}}

@inproceedings{Heittola2020,
    author = "Heittola, Toni and Mesaros, Annamaria and Virtanen, Tuomas",
    title = "Acoustic scene classification in DCASE 2020 Challenge: generalization across devices and low complexity solutions",
    booktitle = "Proceedings of the Detection and Classification of Acoustic Scenes and Events 2020 Workshop (DCASE2020)",
    year = "2020",
    pages = "56--60",
    abstract = "This paper presents the details of Task 1: Acoustic Scene Classification in the DCASE 2020 Challenge. The task consists of two subtasks: classification of data from multiple devices, requiring good generalization properties, and classification using low-complexity solutions. Here we describe the datasets and baseline systems. After the challenge submission deadline, challenge results and analysis of the submissions will be added.",
    url = "https://arxiv.org/abs/2005.14623"
}


@article{warden2018speech,
  title={Speech commands: A dataset for limited-vocabulary speech recognition},
  author={Warden, Pete},
  journal={arXiv preprint arXiv:1804.03209},
  year={2018}
}

@inproceedings{amir2017low,
  title={A low power, fully event-based gesture recognition system},
  author={Amir, Arnon and Taba, Brian and Berg, David and Melano, Timothy and McKinstry, Jeffrey and Di Nolfo, Carmelo and Nayak, Tapan and Andreopoulos, Alexander and Garreau, Guillaume and Mendoza, Marcela and others},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={7243--7252},
  year={2017}
}



@article{Cramer22heidelberg,
	doi = {10.1109/tnnls.2020.3044364},
  
	url = {https://doi.org/10.1109%2Ftnnls.2020.3044364},
  
	year = 2022,
	month = {jul},
  
	publisher = {Institute of Electrical and Electronics Engineers ({IEEE})},
  
	volume = {33},
  
	number = {7},
  
	pages = {2744--2757},
  
	author = {Benjamin Cramer and Yannik Stradmann and Johannes Schemmel and Friedemann Zenke},
  
	title = {The Heidelberg Spiking Data Sets for the Systematic Evaluation of Spiking Neural Networks},
  
	journal = {{IEEE} Transactions on Neural Networks and Learning Systems}
}




@misc{massa2021efficient,
      title={An Efficient Spiking Neural Network for Recognizing Gestures with a DVS Camera on the Loihi Neuromorphic Processor}, 
      author={Riccardo Massa and Alberto Marchisio and Maurizio Martina and Muhammad Shafique},
      year={2021},
      eprint={2006.09985},
      archivePrefix={arXiv},
      primaryClass={cs.NE}
}

@misc{fang2021incorporating,
      title={Incorporating Learnable Membrane Time Constant to Enhance Learning of Spiking Neural Networks}, 
      author={Wei Fang and Zhaofei Yu and Yanqi Chen and Timothee Masquelier and Tiejun Huang and Yonghong Tian},
      year={2021},
      eprint={2007.05785},
      archivePrefix={arXiv},
      primaryClass={cs.NE}
}

@misc{stewart2020online,
      title={Online Few-shot Gesture Learning on a Neuromorphic Processor}, 
      author={Kenneth Stewart and Garrick Orchard and Sumit Bam Shrestha and Emre Neftci},
      year={2020},
      eprint={2008.01151},
      archivePrefix={arXiv},
      primaryClass={cs.NE}
}

@inproceedings{tao2020fscil,
  author = {Tao, Xiaoyu and Hong, Xiaopeng and Chang, Xinyuan and Dong, Songlin and Wei, Xing and Gong, Yihong},
  title = {Few-Shot Class-Incremental Learning},
  booktitle = {Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  year = {2020}
}

@inproceedings{mazumder21mswc,
 author = {Mazumder, Mark and Chitlangia, Sharad and Banbury, Colby and Kang, Yiping and Ciro, Juan and Achorn, Keith and Galvez, Daniel and Sabini, Mark and Mattson, Peter and Kanter, David and Diamos, Greg and Warden, Pete and Meyer, Josh and Janapa Reddi, Vijay},
 booktitle = {Proceedings of the Neural Information Processing Systems Track on Datasets and Benchmarks},
 editor = {J. Vanschoren and S. Yeung},
 pages = {},
 publisher = {Curran},
 title = {Multilingual Spoken Words Corpus},
 url = {https://datasets-benchmarks-proceedings.neurips.cc/paper_files/paper/2021/file/fe131d7f5a6b38b23cc967316c13dae2-Paper-round2.pdf},
 volume = {1},
 year = {2021}
}

@inproceedings{Perot2020,
author = {Perot, Etienne and de Tournemire, Pierre and Nitti, Davide and Masci, Jonathan and Sironi, Amos},
title = {Learning to Detect Objects with a 1 Megapixel Event Camera},
year = {2020},
booktitle = {Proceedings of the 34th International Conference on Neural Information Processing Systems},
series = {NIPS'20}
}

@misc{makin-dataset,
  author = {O'{D}oherty, Joseph E. and Cardoso, Mariana M. B. and Makin, Joseph G. and Sabes, Philip N.},
  title  = {Nonhuman Primate Reaching with Multichannel Sensorimotor Cortex electrophysiology},
  doi	= {10.5281/zenodo.788569},
  url	= {https://doi.org/10.5281/zenodo.788569},
  month  = may,
  year   = {2017}
}



@ARTICLE{Gallego2022,
  author={Gallego, Guillermo and Delbrück, Tobi and Orchard, Garrick and Bartolozzi, Chiara and Taba, Brian and Censi, Andrea and Leutenegger, Stefan and Davison, Andrew J. and Conradt, Jörg and Daniilidis, Kostas and Scaramuzza, Davide},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence}, 
  title={Event-Based Vision: A Survey}, 
  year={2022},
  volume={44},
  number={1},
  pages={154-180},
  doi={10.1109/TPAMI.2020.3008413}}






--------------------------------

@article{He:2021tm,
author = {He, Jiayuan and Hua, Wenmian and Lu, Yi Shan and Maleki, Sepideh and Yang, Yihang and Pingali, Keshav and Manohar, Rajit},
title = {{interact: An Interactive Design Environment for Asynchronous Logic}},
journal = {Woset-workshop},
year = {2021},
pages = {1--4}
}

@article{jones2018stop,
  title={How to stop data centres from gobbling up the world’s electricity},
  author={Jones, Nicola and others},
  journal={Nature},
  volume={561},
  number={7722},
  pages={163--166},
  year={2018},
  publisher={Springer Science and Business Media LLC}
}

@misc{fabrizio30:online,
author = {},
title = {fabrizio-ottati/awesome-neuromorphic-hw: A list of papers, docs, codes about neuromorphic hardware. This repo aims at providing the info for neuromorphic hardware research, we are continuously improving the project. Welcome to PR the works (papers, repositories) that are missed by the repo.},
howpublished = {\url{https://github.com/fabrizio-ottati/awesome-neuromorphic-hw}},
month = {},
year = {},
note = {(Accessed on 04/03/2023)}
}

@article{mattson2020mlperf,
  title={Mlperf training benchmark},
  author={Mattson, Peter and Cheng, Christine and Diamos, Gregory and Coleman, Cody and Micikevicius, Paulius and Patterson, David and Tang, Hanlin and Wei, Gu-Yeon and Bailis, Peter and Bittorf, Victor and others},
  journal={Proceedings of Machine Learning and Systems},
  volume={2},
  pages={336--349},
  year={2020}
}


@article{Ataei:2021jx,
author = {Ataei, Samira and Hua, Wenmian and Yang, Yihang and Manohar, Rajit and Lu, Yi Shan and He, Jiayuan and Maleki, Sepideh and Pingali, Keshav},
title = {{An Open-Source {EDA} Flow for Asynchronous Logic}},
journal = {IEEE Design and Test},
year = {2021},
volume = {38},
number = {2},
pages = {27--37},
month = apr,
affiliation = {The University of Texas at Austin, Austin, United States},
doi = {10.1109/MDAT.2021.3051334},
uri = {\url{papers3://publication/doi/10.1109/MDAT.2021.3051334}}
}


@article{Merolla:2014fj,
author = {Merolla, P A and Arthur, John V and Alvarez-Icaza, R and Cassidy, A S and Sawada, J and Akopyan, F. and Jackson, B L and Imam, N. and Guo, C and Nakamura, Y and Brezzo, B. and Vo, I and Esser, Steven K and Appuswamy, R and Taba, B and Amir, A and Flickner, M D and Risk, W P and Manohar, Rajit and Modha, Dharmendra S},
title = {{A million spiking-neuron integrated circuit with a scalable communication network and interface}},
journal = {Science},
year = {2014},
volume = {345},
number = {6197},
pages = {668--673},
month = aug,
doi = {10.1126/science.1254642}
}

@inproceedings{Cassidy:2014ws,
author = {Cassidy, Andrew S and Alvarez-Icaza, Rodrigo and Akopyan, Filipp and Sawada, Jun and Arthur, John V and Merolla, Paul A and Datta, Pallab and Tallada, Marc Gonzalez and Taba, Brian and Andreopoulos, Alexander and Amir, Arnon and Esser, Steven K and Kusnitz, Jeff and Appuswamy, Rathinakumar and Haymes, Chuck and Brezzo, Bernard and Moussalli, Roger and Bellofatto, Ralph and Baks, Christian and Mastro, Michael and Schleupen, Kai and Cox, Charles E and Inoue, Ken and Millman, Steve and Imam, Nabil and McQuinn, Emmett and Nakamura, Yutaka Y and Vo, Ivan and Guo, Chen and Nguyen, Don and Lekuch, Scott and Asaad, Sameh and Friedman, Daniel and Jackson, Bryan L and Flickner, Myron D and Risk, William P and Manohar, Rajit and Modha, Dharmendra S},
title = {{Real-time scalable cortical computing at 46 giga-synaptic {OPS/watt} with 100X speedup in time-to-solution and 100,000X  reduction in energy-to-solution}},
booktitle = {Proceedings of the International Conference for High Performance Computing, Networking, Storage and Analysis (SC'14)},
year = {2014},
pages = {27--37},
publisher = {~IEEE Press}
}

@article{Davies:2018jn,
author = {Davies, Mike and Srinivasa, Narayan and Lin, Tsung-Han and Chinya, Gautham and Cao, Yongqiang and Choday, Sri Harsha and Dimou, Georgios and Joshi, Prasad and Imam, Nabil and Jain, Shweta and Liao, Yuyun and Lin, Chit-Kwan and Lines, Andrew and Liu, Ruokun and Mathaikutty, Deepak and McCoy, Steven and Paul, Arnab and Tse, Jonathan and Venkataramanan, Guruguhanathan and Weng, Yi-Hsin and Wild, Andreas and Yang, Yoonseok and Wang, Hong},
title = {{Loihi: A Neuromorphic Manycore Processor with On-Chip Learning}},
journal = {IEEE Micro},
year = {2018},
volume = {38},
number = {1},
pages = {82--99},
month = feb,
publisher = {IEEE},
doi = {10.1109/MM.2018.112130359}}


@article{Cassidy:2013vm,
author = {Cassidy, Andrew S and Georgiou, Julius and Andreou, Andreas G},
title = {{Design of silicon brains in the {nano-CMOS era:} spiking neurons, learning synapses and neural architecture optimization}},
journal = {Neural Networks},
year = {2013},
volume = {45},
pages = {4--26},
month = jun,
doi = {10.1016/j.neunet.2013.05.011}
}

@article{Cassidy:2012if,
author = {Cassidy, Andrew S and Andreou, Andreas G},
title = {{Beyond {Amdahl's Law}: an objective function that links multiprocessor performance gains to delay and energy}},
journal = {IEEE Transactions on Computers},
year = {2012},
volume = {61},
number = {8},
pages = {1110--1126},
month = aug,
doi = {10.1109/TC.2011.169}
}

@article{Mead:1990hw,
author = {Mead, Carver A},
title = {{Neuromorphic electronic systems}},
journal = {Proceedings of the IEEE},
year = {1990},
volume = {78},
number = {10},
pages = {1629--1636},
doi = {10.1109/5.58356}
}

@inproceedings{Bohus:2017fs,
author = {Bohus, Dan and Andrist, Sean and Jalobeanu, Mihai},
title = {{Rapid development of multimodal interactive systems: a demonstration of platform for situated intelligence}},
booktitle = {the 19th ACM International Conference},
year = {2017},
pages = {493--494},
publisher = {ACM Press},
address = {New York, New York, USA},
doi = {10.1145/3136755.3143021},
isbn = {9781450355438},
url = {http://dl.acm.org/citation.cfm?doid=3136755.3143021}
}

@article{Bekolay:2014fl,
author = {Bekolay, T and Bergstra, J and Hunsberger, E},
title = {{Nengo: a {Python} tool for building large-scale functional brain models}},
journal = {Frontiers in Neuroinformatics},
year = {2014},
volume = {7},
number = {48},
pages = {1--13},
month = jan,
doi = {10.3389/fninf.2013.00048/abstract}
}

@inproceedings{FIschl:2019wx,
author = {Fischl, Kate D and Cellon, Adam B and Stewart, Terrence C and Horiuchi, Timothy K and Andreou, Andreas G},
title = {{Socio-Emotional Robot with Distributed Multi-Platform Neuromorphic Processing}},
booktitle = {53rd Annual Conference on Information Sciences and Systems (CISS)},
year = {2019},
pages = {1--6},
month = jan
}

@inproceedings{Mendat2023,
  title = {A {{RISC-V Neuromorphic Micro-Controller Unit}} ({{vMCU}}) with an Event Based Physical Interface, Micro-Architectural Units and Accelerator for Low Latency Machine Perception and Intelligence at the Edge.},
  booktitle = {2023 {{International Sysmposium Circuits}} and {{Systems}}},
  author = {Mendat, Daniel R and Sengupta, Jonah P and Tognetti, Gaspar and Villemur, Martin and Andreou, Andreas G},
  date = {2023}
}

@inproceedings{Molin2022,
  title = {Edge Super Compute \textendash{} a System-on-Chip for High Performance Edge Computing},
  booktitle = {{{GOMAC}}},
  author = {Molin, Jamal Lottier and Andreou, Andreas G},
  year = {2022},
  pages = {1--5}
}



@article{sainath2015convolutional,
  title={Convolutional neural networks for small-footprint keyword spotting},
  author={Sainath, Tara and Parada, Carolina},
  year={2015}
}


@article{choi2019temporal,
  title={Temporal convolution for real-time keyword spotting on mobile devices},
  author={Choi, Seungwoo and Seo, Seokjun and Shin, Beomjun and Byun, Hyeongmin and Kersner, Martin and Kim, Beomsu and Kim, Dongyoung and Ha, Sungjoo},
  journal={arXiv preprint arXiv:1904.03814},
  year={2019}
}


@inproceedings{chen2015query,
  title={Query-by-example keyword spotting using long short-term memory networks},
  author={Chen, Guoguo and Parada, Carolina and Sainath, Tara N},
  booktitle={2015 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={5236--5240},
  year={2015},
  organization={IEEE}
}


@article{rayner2010spoken,
  title={Spoken dialogue application in space: The Clarissa procedure browser},
  author={Rayner, Manny and Hockey, Beth Ann and Renders, Jean-Michel and Chatzichrisafis, Nikos and Farrell, Kim},
  journal={Speech Technology: Theory and Applications},
  pages={221--250},
  year={2010},
  publisher={Springer}
}


@inproceedings{tan2019vehicle,
  title={An in-vehicle keyword spotting system with multi-source fusion for vehicle applications},
  author={Tan, Yue and Zheng, Kan and Lei, Lei},
  booktitle={2019 IEEE Wireless Communications and Networking Conference (WCNC)},
  pages={1--6},
  year={2019},
  organization={IEEE}
}

 @ARTICLE{GT_neuron,
  author={S. Brink and S. Nease and P. Hasler and et. al.},
  journal={IEEE Transactions on Biomedical Circuits and Systems},
  title={A Learning-Enabled Neuron Array IC Based Upon Transistor Channel Models of Biological Phenomena},
  year={2013},
  volume={7},
  number={1},
  pages={71-81},
  }

  @ARTICLE{FPAA_SOC,
  author={S. George and S. Kim and S. Shah and et. al.},
  journal={IEEE Transactions on VLSI},
  title={A Programmable and Configurable Mixed-Mode FPAA SoC
},
  year={2016},
  volume={24},
  number={6},
  pages={2253-61},
  }

  @ARTICLE{FPAA_Basu,
  author={A. Basu and S. Brink and C. Schlottmann and et. al.},
  journal={IEEE Journal of Solid-State Circuits},
  title={A floating-gate-based field-programmable analog array},
  year={2010},
  volume={45},
  number={9},
  pages={1781-94},
  }
  @ARTICLE{FPAA_Neural,
  author={A. Basu and S. Ramakrishnan and C. Petre and et. al.},
  journal={IEEE Trans. On Biomedical Circuits and Systems},
  title={Neural Dynamics in Reconfigurable Silicon},
  year={2010},
  volume={4},
  number={5},
  pages={311-319},
  }

 @ARTICLE{FPAA_dendrites,
  author={A. Basu and S. Brink and C. Schlottmann and et. al.},
  journal={IEEE Transactions on Biomedical Circuits and Systems},
  title={Neuron array with plastic synapses and programmable dendrites},
  year={2013},
  volume={7},
  number={5},
  pages={631-642},
  }

@ARTICLE{Yi_decoder,
  author={Y. Chen and E. Yao and A. Basu},
  journal={IEEE Transactions on Biomedical Circuits and Systems},
  title={A 128-channel extreme learning machine-based neural decoder for brain machine interfaces},
  year={2015},
  volume={10},
  number={3},
  pages={679-692},
  doi={10.1109/TBCAS.2019.2944486}
}


  @ARTICLE{ShoebiBMI,
  author={Shaikh, Shoeb and So, Rosa and Sibindi, Tafadzwa and Libedinsky, Camilo and Basu, Arindam},
  journal={IEEE Transactions on Biomedical Circuits and Systems},
  title={Towards Intelligent Intracortical BMI (i$^2$BMI): Low-Power Neuromorphic Decoders That Outperform Kalman Filters},
  year={2019},
  volume={13},
  number={6},
  pages={1615-1624},
  doi={10.1109/TBCAS.2019.2944486}}

@ARTICLE{closedloop-terry,
AUTHOR={Stewart, Terrence C. and DeWolf, Travis and Kleinhans, Ashley and Eliasmith, Chris},   
TITLE={Closed-Loop Neuromorphic Benchmarks}, 	 
JOURNAL={Frontiers in Neuroscience}, 	 
VOLUME={9},      	 
YEAR={2015}, 	 
URL={https://www.frontiersin.org/articles/10.3389/fnins.2015.00464},  	 
DOI={10.3389/fnins.2015.00464},
 }

 @ARTICLE{closedloop-andre,
AUTHOR={Milde, Moritz B. and Afshar, Saeed and Xu, Ying and Marcireau, Alexandre and Joubert, Damien and Ramesh, Bharath and Bethi, Yeshwanth and Ralph, Nicholas O. and El Arja, Sami and Dennler, Nik and van Schaik, André and Cohen, Gregory},   
TITLE={Neuromorphic Engineering Needs Closed-Loop Benchmarks}, 	 
JOURNAL={Frontiers in Neuroscience}, 	 
VOLUME={16},      	 
YEAR={2022},      	 
DOI={10.3389/fnins.2022.813555},
 }



 @ARTICLE{makin-paper,
AUTHOR={Makin, J. G. and O'Doherty, J. E. and Cardoso, M. M. B and Sabes, P.N.},   
TITLE={Superior arm-movement decoding from cortex with a new, unsupervised-learning algorithm}, 	 
JOURNAL={J. Neural Eng.}, 	 
VOLUME={15},
number={2},
YEAR={2018},      	 
DOI={10.1088/1741-2552/aa9e95},
 }


@inproceedings{Ilya2014,
author = {I. Sutskever and O. Vinyals and Q. V. Le},
title = {Sequence to Sequence Learning with Neural Networks
},
year = {2014},
booktitle = {Proceedings of the 27th International Conference on Neural Information Processing Systems},
series = {NIPS'14}
}

 
@misc{DatasetObjectDetection,
  title = {1Megapixel automative object detection dataset},
  howpublished = {\url{https://www.prophesee.ai/2020/11/24/automotive-megapixel-event-based-dataset/ }},
}


@InProceedings{LinCOCO_2014,
author="Lin, Tsung-Yi and Maire, Michael and Belongie, Serge and Hays, James and Perona, Pietro and Ramanan, Deva
and Doll{\'a}r, Piotr and Zitnick, C. Lawrence",
title="Microsoft {COCO}: Common Objects in Context",
booktitle="Computer Vision -- ECCV 2014",
year="2014",
pages="740--755",
}


@misc{code_Coco,
  title = {{COCO} API},
  howpublished = {\url{https://github.com/cocodataset/cocoapi}},
}

@article{li2022wearable,
  title={Wearable-based Human Activity Recognition with Spatio-Temporal Spiking Neural Networks},
  author={Li, Yuhang and Yin, Ruokai and Park, Hyoungseob and Kim, Youngeun and Panda, Priyadarshini},
  journal={arXiv preprint arXiv:2212.02233},
  year={2022}
}

@article{roy2019towards,
  title={Towards spike-based machine intelligence with neuromorphic computing},
  author={Roy, Kaushik and Jaiswal, Akhilesh and Panda, Priyadarshini},
  journal={Nature},
  volume={575},
  number={7784},
  pages={607--617},
  year={2019},
  publisher={Nature Publishing Group UK London}
}



@INPROCEEDINGS{frenkel2022,
  author={Frenkel, Charlotte and Indiveri, Giacomo},
  booktitle={2022 IEEE International Solid- State Circuits Conference (ISSCC)}, 
  title={ReckOn: A 28nm Sub-mm2 Task-Agnostic Spiking Recurrent Neural Network Processor Enabling On-Chip Learning over Second-Long Timescales}, 
  year={2022},
  volume={65},
  number={},
  pages={1-3},
  doi={10.1109/ISSCC42614.2022.9731734}}

@inproceedings{guthaus2016openram,
  title={OpenRAM: An open-source memory compiler},
  author={Guthaus, Matthew R and Stine, James E and Ataei, Samira and Chen, Brian and Wu, Bin and Sarwar, Mehedi},
  booktitle={2016 IEEE/ACM International Conference on Computer-Aided Design (ICCAD)},
  pages={1--6},
  year={2016},
  organization={IEEE}
}


@INBOOK{bos2022,
  author={Bos, Hannah and Muir, Dylan Richard},
  booktitle={Embedded Artificial Intelligence: Devices, Embedded Systems, and Industrial Applications}, 
  title={7. Sub-mW Neuromorphic SNN Audio Processing Applications with Rockpool and Xylo}, 
  year={2022},
  volume={},
  number={},
  pages={69-78},
  url={https://ieeexplore.ieee.org/document/9967462}}

@inproceedings{kim2022rate,
  title={Rate coding or direct coding: Which one is better for accurate, robust, and energy-efficient spiking neural networks?},
  author={Kim, Youngeun and Park, Hyoungseob and Moitra, Abhishek and Bhattacharjee, Abhiroop and Venkatesha, Yeshwanth and Panda, Priyadarshini},
  booktitle={ICASSP 2022-2022 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={71--75},
  year={2022},
  organization={IEEE}
}

@article{sun2022intelligence,
  title={Intelligence Processing Units Accelerate Neuromorphic Learning},
  author={Sun, Pao-Sheng Vincent and Titterton, Alexander and Gopiani, Anjlee and Santos, Tim and Basu, Arindam and Lu, Wei D and Eshraghian, Jason K},
  journal={arXiv preprint arXiv:2211.10725},
  year={2022}
}


@ARTICLE{nest2007,
  author  = {Marc-Oliver Gewaltig and Markus Diesmann},
  title   = {NEST (NEural Simulation Tool)},
  journal = {Scholarpedia},
  year    = {2007},
  volume  = {2},
  pages   = {1430},
  number  = {4}
}

@article{zhu2023spikegpt,
  title={SpikeGPT: Generative Pre-trained Language Model with Spiking Neural Networks},
  author={Zhu, Rui-Jie and Zhao, Qihang and Eshraghian, Jason K},
  journal={arXiv preprint arXiv:2302.13939},
  year={2023}
}


@misc{rockpool2019,
  author       = {Muir, Dylan and
                  Bauer, Felix and
                  Weidel, Philipp},
  title        = {Rockpool Documentaton},
  year         = 2019,
  publisher    = {Zenodo},
  doi          = {10.5281/zenodo.3773845}
}
@article{Stimberg2019,
    title = {Brian 2, an intuitive and efficient neural simulator},
    volume = {8},
    issn = {2050-084X},
    doi = {10.7554/eLife.47314},
    journal = {eLife},
    author = {Stimberg, Marcel and Brette, Romain and Goodman, Dan FM},
    editor = {Skinner, Frances K},
    month = aug,
    year = {2019},
    pages = {e47314}
}

@misc{norse2021,
  author       = {Pehle, Christian and
                  Pedersen, Jens Egholm},
  title        = {{Norse -  A deep learning library for spiking 
                   neural networks}},
  month        = jan,
  year         = 2021,
  note         = {Documentation: https://norse.ai/docs/},
  publisher    = {Zenodo},
  version      = {0.0.7},
  doi          = {10.5281/zenodo.4422025},
  url          = {https://doi.org/10.5281/zenodo.4422025}
}



@ARTICLE{bindsnet2018,
	AUTHOR={Hazan, Hananel and Saunders, Daniel J. and Khan, Hassaan and Patel, Devdhar and Sanghavi, Darpan T. and Siegelmann, Hava T. and Kozma, Robert},   
	TITLE={BindsNET: A Machine Learning-Oriented Spiking Neural Networks Library in Python},      
	JOURNAL={Frontiers in Neuroinformatics},      
	VOLUME={12},      
	PAGES={89},     
	YEAR={2018}, 
	URL={https://www.frontiersin.org/article/10.3389/fninf.2018.00089},       
	DOI={10.3389/fninf.2018.00089},      
	ISSN={1662-5196},
}
@article{Merolla2014,
author = {Paul A. Merolla  and John V. Arthur  and Rodrigo Alvarez-Icaza  and Andrew S. Cassidy  and Jun Sawada  and Filipp Akopyan  and Bryan L. Jackson  and Nabil Imam  and Chen Guo  and Yutaka Nakamura  and Bernard Brezzo  and Ivan Vo  and Steven K. Esser  and Rathinakumar Appuswamy  and Brian Taba  and Arnon Amir  and Myron D. Flickner  and William P. Risk  and Rajit Manohar  and Dharmendra S. Modha },
title = {A million spiking-neuron integrated circuit with a scalable communication network and interface},
journal = {Science},
volume = {345},
number = {6197},
pages = {668-673},
year = {2014},
doi = {10.1126/science.1254642},
URL = {https://www.science.org/doi/abs/10.1126/science.1254642},
eprint = {https://www.science.org/doi/pdf/10.1126/science.1254642},
}

@inproceedings{bhattacharjee2022examining,
  title={Examining the robustness of spiking neural networks on non-ideal memristive crossbars},
  author={Bhattacharjee, Abhiroop and Kim, Youngeun and Moitra, Abhishek and Panda, Priyadarshini},
  booktitle={Proceedings of the ACM/IEEE International Symposium on Low Power Electronics and Design},
  pages={1--6},
  year={2022}
}

﻿@Article{Pei2019,
author={Pei, Jing and Deng, Lei and Song, Sen and Zhao, Mingguo and Zhang, Youhui and Wu, Shuang and Wang, Guanrui and Zou, Zhe and Wu, Zhenzhi and He, Wei and Chen, Feng and Deng, Ning and Wu, Si and Wang, Yu and Wu, Yujie and Yang, Zheyu and Ma, Cheng and Li, Guoqi and Han, Wentao and Li, Huanglong and Wu, Huaqiang and Zhao, Rong and Xie, Yuan and Shi, Luping},
title={Towards artificial general intelligence with hybrid Tianjic chip architecture},
journal={Nature},
year={2019},
month={Aug},
day={01},
volume={572},
number={7767},
pages={106-111},
issn={1476-4687},
doi={10.1038/s41586-019-1424-8},
url={https://doi.org/10.1038/s41586-019-1424-8}
}

﻿@Article{Mehonic2022,
author={Mehonic, A. and Kenyon, A. J.},
title={Brain-inspired computing needs a master plan},
journal={Nature},
year={2022},
month={Apr},
day={01},
volume={604},
number={7905},
pages={255-260},
abstract={New computing technologies inspired by the brain promise fundamentally different ways to process information with extreme energy efficiency and the ability to handle the avalanche of unstructured and noisy data that we are generating at an ever-increasing rate. To realize this promise requires a brave and coordinated plan to bring together disparate research communities and to provide them with the funding, focus and support needed. We have done this in the past with digital technologies; we are in the process of doing it with quantum technologies; can we now do it for brain-inspired computing?},
issn={1476-4687},
doi={10.1038/s41586-021-04362-w},
url={https://doi.org/10.1038/s41586-021-04362-w}
}

@article{kim2022beyond,
  title={Beyond classification: Directly training spiking neural networks for semantic segmentation},
  author={Kim, Youngeun and Chough, Joshua and Panda, Priyadarshini},
  journal={Neuromorphic Computing and Engineering},
  volume={2},
  number={4},
  pages={044015},
  year={2022},
  publisher={IOP Publishing}
}

@inproceedings{li2022neuromorphic,
  title={Neuromorphic data augmentation for training spiking neural networks},
  author={Li, Yuhang and Kim, Youngeun and Park, Hyoungseob and Geller, Tamar and Panda, Priyadarshini},
  booktitle={Computer Vision--ECCV 2022: 17th European Conference, Tel Aviv, Israel, October 23--27, 2022, Proceedings, Part VII},
  pages={631--649},
  year={2022},
  organization={Springer}
}

@inproceedings{eshraghian2022navigating,
  title={Navigating Local Minima in Quantized Spiking Neural Networks},
  author={Eshraghian, Jason K and Lammie, Corey and Azghadi, Mostafa Rahimi and Lu, Wei D},
  booktitle={2022 IEEE 4th International Conference on Artificial Intelligence Circuits and Systems (AICAS)},
  pages={352--355},
  year={2022},
  organization={IEEE}
}


@article{panda2017asp,
  title={Asp: Learning to forget with adaptive synaptic plasticity in spiking neural networks},
  author={Panda, Priyadarshini and Allred, Jason M and Ramanathan, Shriram and Roy, Kaushik},
  journal={IEEE Journal on Emerging and Selected Topics in Circuits and Systems},
  volume={8},
  number={1},
  pages={51--64},
  year={2017},
  publisher={IEEE}
}




@ARTICLE{Ceolini2020,
AUTHOR={Ceolini, Enea and Frenkel, Charlotte and Shrestha, Sumit Bam and Taverni, Gemma and Khacef, Lyes and Payvand, Melika and Donati, Elisa},
TITLE={Hand-Gesture Recognition Based on EMG and Event-Based Camera Sensor Fusion: A Benchmark in Neuromorphic Computing},
JOURNAL={Frontiers in Neuroscience},
VOLUME={14},
YEAR={2020},
URL={https://www.frontiersin.org/articles/10.3389/fnins.2020.00637},
DOI={10.3389/fnins.2020.00637},
ISSN={1662-453X},
}

@article{Ma2022,
author = {Songchen Ma  and Jing Pei  and Weihao Zhang  and Guanrui Wang  and Dahu Feng  and Fangwen Yu  and Chenhang Song  and Huanyu Qu  and Cheng Ma  and Mingsheng Lu  and Faqiang Liu  and Wenhao Zhou  and Yujie Wu  and Yihan Lin  and Hongyi Li  and Taoyi Wang  and Jiuru Song  and Xue Liu  and Guoqi Li  and Rong Zhao  and Luping Shi },
title = {Neuromorphic computing chip with spatiotemporal elasticity for multi-intelligent-tasking robots},
journal = {Science Robotics},
volume = {7},
number = {67},
pages = {eabk2948},
year = {2022},
doi = {10.1126/scirobotics.abk2948},
URL = {https://www.science.org/doi/abs/10.1126/scirobotics.abk2948},
eprint = {https://www.science.org/doi/pdf/10.1126/scirobotics.abk2948},
}

@ARTICLE{Aitsam2022,
  author={Aitsam, Muhammad and Davies, Sergio and Di Nuovo, Alessandro},
  journal={IEEE Access}, 
  title={Neuromorphic Computing for Interactive Robotics: A Systematic Review}, 
  year={2022},
  volume={10},
  number={},
  pages={122261-122279},
  doi={10.1109/ACCESS.2022.3219440}}



@article{Ji2020,
author = {Ji, Xinglong and Zhao, Xinyu and Tan, Mei Chee and Zhao, Rong},
title = {Artificial Perception Built on Memristive System: Visual, Auditory, and Tactile Sensations},
journal = {Advanced Intelligent Systems},
volume = {2},
number = {3},
pages = {1900118},
keywords = {artificial perception, auditory sensation, memristive systems, neuromorphic systems, sensors, tactile sensation, visual sensation},
doi = {https://doi.org/10.1002/aisy.201900118},
url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/aisy.201900118},
eprint = {https://onlinelibrary.wiley.com/doi/pdf/10.1002/aisy.201900118},
year = {2020}
}

@article{yan2021comparing,
doi = {10.1088/2634-4386/abf150},
url = {https://dx.doi.org/10.1088/2634-4386/abf150},
year = {2021},
month = {jul},
publisher = {IOP Publishing},
volume = {1},
number = {1},
pages = {014002},
author = {Yexin Yan and Terrence C Stewart and Xuan Choo and Bernhard Vogginger and Johannes Partzsch and Sebastian Höppner and Florian Kelber and Chris Eliasmith and Steve Furber and Christian Mayr},
title = {Comparing Loihi with a SpiNNaker 2 prototype on low-latency keyword spotting and adaptive robotic control},
journal = {Neuromorphic Computing and Engineering },
}

@inproceedings{blouw2019,
author = {Blouw, Peter and Choo, Xuan and Hunsberger, Eric and Eliasmith, Chris},
title = {Benchmarking Keyword Spotting Efficiency on Neuromorphic Hardware},
year = {2019},
isbn = {9781450361231},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3320288.3320304},
doi = {10.1145/3320288.3320304},
booktitle = {Proceedings of the 7th Annual Neuro-Inspired Computational Elements Workshop},
articleno = {1},
numpages = {8},
keywords = {keyword spotting, spiking neural networks, speech recognition, neuromorphic computing, machine learning},
location = {Albany, NY, USA},
series = {NICE '19}
}

@article{sandarmirskaya2022,
author = {Yulia Sandamirskaya  and Mohsen Kaboli  and Jorg Conradt  and Tansu Celikel },
title = {Neuromorphic computing hardware and neural architectures for robotics},
journal = {Science Robotics},
volume = {7},
number = {67},
pages = {eabl8419},
year = {2022},
doi = {10.1126/scirobotics.abl8419},
URL = {https://www.science.org/doi/abs/10.1126/scirobotics.abl8419},
eprint = {https://www.science.org/doi/pdf/10.1126/scirobotics.abl8419},}

@article{liang2021h2learn,
  title={H2learn: High-efficiency learning accelerator for high-accuracy spiking neural networks},
  author={Liang, Ling and Qu, Zheng and Chen, Zhaodong and Tu, Fengbin and Wu, Yujie and Deng, Lei and Li, Guoqi and Li, Peng and Xie, Yuan},
  journal={IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems},
  volume={41},
  number={11},
  pages={4782--4796},
  year={2021},
  publisher={IEEE}
}

@inproceedings{narayanan2020spinalflow,
  title={SpinalFlow: An architecture and dataflow tailored for spiking neural networks},
  author={Narayanan, Surya and Taht, Karl and Balasubramonian, Rajeev and Giacomin, Edouard and Gaillardon, Pierre-Emmanuel},
  booktitle={2020 ACM/IEEE 47th Annual International Symposium on Computer Architecture (ISCA)},
  pages={349--362},
  year={2020},
  organization={IEEE}
}

@article{yin2022sata,
  title={Sata: Sparsity-aware training accelerator for spiking neural networks},
  author={Yin, Ruokai and Moitra, Abhishek and Bhattacharjee, Abhiroop and Kim, Youngeun and Panda, Priyadarshini},
  journal={IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems},
  year={2022},
  publisher={IEEE}
}

@article{moitra2022spikesim,
  title={SpikeSim: An end-to-end Compute-in-Memory Hardware Evaluation Tool for Benchmarking Spiking Neural Networks},
  author={Moitra, Abhishek and Bhattacharjee, Abhiroop and Kuang, Runcong and Krishnan, Gokul and Cao, Yu and Panda, Priyadarshini},
  journal={arXiv preprint arXiv:2210.12899},
  year={2022}
}

@article{zhou2022gradient,
  title={Gradient-Based Neuromorphic Learning on Dynamical RRAM Arrays},
  author={Zhou, Peng and Choi, Dong-Uk and Lu, Wei D and Kang, Sung-Mo and Eshraghian, Jason K},
  journal={IEEE Journal on Emerging and Selected Topics in Circuits and Systems},
  volume={12},
  number={4},
  pages={888--897},
  year={2022},
  publisher={IEEE}
}



@ARTICLE{Moradi2018,
  author={Moradi, Saber and Qiao, Ning and Stefanini, Fabio and Indiveri, Giacomo},
  journal={IEEE Transactions on Biomedical Circuits and Systems}, 
  title={A Scalable Multicore Architecture With Heterogeneous Memory Structures for Dynamic Neuromorphic Asynchronous Processors (DYNAPs)}, 
  year={2018},
  volume={12},
  number={1},
  pages={106-122},
  doi={10.1109/TBCAS.2017.2759700}}

@misc{Mayr2019,
      title={SpiNNaker 2: A 10 Million Core Processor System for Brain Simulation and Machine Learning}, 
      author={Christian Mayr and Sebastian Hoeppner and Steve Furber},
      year={2019},
      eprint={1911.02385},
      archivePrefix={arXiv},
      primaryClass={cs.ET}
}

@INPROCEEDINGS{Meier2015,
  author={Meier, Karlheinz},
  booktitle={2015 IEEE International Electron Devices Meeting (IEDM)}, 
  title={A mixed-signal universal neuromorphic computing system}, 
  year={2015},
  volume={},
  number={},
  pages={4.6.1-4.6.4},
  doi={10.1109/IEDM.2015.7409627}}

@misc{LocalPlasticity22,
     	title={Spike-based local synaptic plasticity: A survey of computational models and neuromorphic circuits}, 
   	author={Lyes Khacef and Philipp Klein and Matteo Cartiglia and Arianna Rubino and Giacomo Indiveri and Elisabetta Chicca},
      year={2022},
      eprint={2209.15536},
      archivePrefix={arXiv},
      primaryClass={cs.NE}
}

@ARTICLE{Ostrau2022,
  
AUTHOR={Ostrau, Christoph and Klarhorst, Christian and Thies, Michael and Rückert, Ulrich},   
	 
TITLE={Benchmarking Neuromorphic Hardware and Its Energy Expenditure},      
	
JOURNAL={Frontiers in Neuroscience},      
	
VOLUME={16},           
	
YEAR={2022},      
	  
URL={https://www.frontiersin.org/articles/10.3389/fnins.2022.873935},       
	
DOI={10.3389/fnins.2022.873935},      
	
ISSN={1662-453X},   
   
ABSTRACT={We propose and discuss a platform overarching benchmark suite for neuromorphic hardware. This suite covers benchmarks from low-level characterization to high-level application evaluation using benchmark specific metrics. With this rather broad approach we are able to compare various hardware systems including mixed-signal and fully digital neuromorphic architectures. Selected benchmarks are discussed and results for several target platforms are presented revealing characteristic differences between the various systems. Furthermore, a proposed energy model allows to combine benchmark performance metrics with energy efficiency. This model enables the prediction of the energy expenditure of a network on a target system without actually having access to it. To quantify the efficiency gap between neuromorphics and the biological paragon of the human brain, the energy model is used to estimate the energy required for a full brain simulation. This reveals that current neuromorphic systems are at least four orders of magnitude less efficient. It is argued, that even with a modern fabrication process, two to three orders of magnitude are remaining. Finally, for selected benchmarks the performance and efficiency of the neuromorphic solution is compared to standard approaches.}
}
 


@article{KULKARNI2021,
title = {Benchmarking the performance of neuromorphic and spiking neural network simulators},
journal = {Neurocomputing},
volume = {447},
pages = {145-160},
year = {2021},
issn = {0925-2312},
doi = {https://doi.org/10.1016/j.neucom.2021.03.028},
url = {https://www.sciencedirect.com/science/article/pii/S0925231221003969},
author = {Shruti R. Kulkarni and Maryam Parsa and J. Parker Mitchell and Catherine D. Schuman},
keywords = {Neuromorphic computers, Spiking neural networks, Neuromorphic simulators, Benchmarking, Neuromorphic computing workloads, High Performance Computing (HPC) systems, Scalable systems},
abstract = {Software simulators play a critical role in the development of new algorithms and system architectures in any field of engineering. Neuromorphic computing, which has shown potential in building brain-inspired energy-efficient hardware, suffers a slow-down in the development cycle due to a lack of flexible and easy-to-use simulators of either neuromorphic hardware itself or of spiking neural networks (SNNs), the type of neural network computation executed on most neuromorphic systems. }
}

@misc{Reddi2020,
      title={MLPerf Inference Benchmark}, 
      author={Vijay Janapa Reddi and Christine Cheng and David Kanter and Peter Mattson and Guenther Schmuelling and Carole-Jean Wu and Brian Anderson and Maximilien Breughe and Mark Charlebois and William Chou and Ramesh Chukka and Cody Coleman and Sam Davis and Pan Deng and Greg Diamos and Jared Duke and Dave Fick and J. Scott Gardner and Itay Hubara and Sachin Idgunji and Thomas B. Jablin and Jeff Jiao and Tom St. John and Pankaj Kanwar and David Lee and Jeffery Liao and Anton Lokhmotov and Francisco Massa and Peng Meng and Paulius Micikevicius and Colin Osborne and Gennady Pekhimenko and Arun Tejusve Raghunath Rajan and Dilip Sequeira and Ashish Sirasao and Fei Sun and Hanlin Tang and Michael Thomson and Frank Wei and Ephrem Wu and Lingjie Xu and Koichi Yamada and Bing Yu and George Yuan and Aaron Zhong and Peizhao Zhang and Yuchen Zhou},
      year={2020},
      eprint={1911.02549},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}
@book{Furber2020, abstract = {20 years in conception and 15 in construction, the SpiNNaker project has delivered the world’s largest neuromorphic computing platform incorporating over a million ARM mobile phone processors and capable of modelling spiking neural networks of the scale of a mouse brain in biological real time. This machine, hosted at the University of Manchester in the UK, is freely available under the auspices of the EU Flagship Human Brain Project. This book tells the story of the origins of the machine, its development and its deployment, and the immense software development effort that has gone into making it openly available and accessible to researchers and students the world over. It also presents exemplar applications from ‘Talk’, a SpiNNaker-controlled robotic exhibit at the Manchester Art Gallery as part of ‘The Imitation Game’, a set of works commissioned in 2016 in honour of Alan Turing, through to a way to solve hard computing problems using stochastic neural networks. The book concludes with a look to the future, and the SpiNNaker-2 machine which is yet to come!}, author = {Steve Furber and Petrut Antoniu Bogdan}, city = {Boston-Delft}, doi = {10.1561/9781680836530}, editor = {Steve Furber and Petrut Antoniu Bogdan}, isbn = {978-1-68083-653-0}, pages = {350}, publisher = {now publishers}, title = {SpiNNaker: A Spiking Neural Network Architecture}, year = {2020}, } 

@ARTICLE{Furber2014,
  author={Furber, Steve B. and Galluppi, Francesco and Temple, Steve and Plana, Luis A.},
  journal={Proceedings of the IEEE}, 
  title={The SpiNNaker Project}, 
  year={2014},
  volume={102},
  number={5},
  pages={652-665},
  doi={10.1109/JPROC.2014.2304638}}

  
@misc{Levy2021,
  author={Levy, Markus},
  title={Innatera's Spiking Neural Processor - Brain-like architecture targets ultra-low power AI}, 
  year={2021},
  journal={Linley Microprocessor Report}}



@ARTICLE{Cramer2022-xi,
  title     = "Surrogate gradients for analog neuromorphic computing",
  author    = "Cramer, Benjamin and Billaudelle, Sebastian and Kanya, Simeon
               and Leibfried, Aron and Gr{\"u}bl, Andreas and Karasenko, Vitali
               and Pehle, Christian and Schreiber, Korbinian and Stradmann,
               Yannik and Weis, Johannes and Schemmel, Johannes and Zenke,
               Friedemann",
  journal   = "Proc. Natl. Acad. Sci. U. S. A.",
  publisher = "National Acad Sciences",
  volume    =  119,
  number    =  4,
  month     =  jan,
  year      =  2022,
  keywords  = "neuromorphic hardware; recurrent neural networks;
               self-calibration; spiking neural networks; surrogate gradients",
  language  = "en"
}
@article{wunderlich2021event,
  title={Event-based backpropagation can compute exact gradients for spiking neural networks},
  author={Wunderlich, Timo C and Pehle, Christian},
  journal={Scientific Reports},
  volume={11},
  number={1},
  pages={12829},
  year={2021},
  publisher={Nature Publishing Group UK London}
}
@inproceedings{schmitt2017neuromorphic,
  title={Neuromorphic hardware in the loop: Training a deep spiking network on the brainscales wafer-scale system},
  author={Schmitt, Sebastian and Kl{\"a}hn, Johann and Bellec, Guillaume and Gr{\"u}bl, Andreas and Guettler, Maurice and Hartel, Andreas and Hartmann, Stephan and Husmann, Dan and Husmann, Kai and Jeltsch, Sebastian and others},
  booktitle={2017 international joint conference on neural networks (IJCNN)},
  pages={2227--2234},
  year={2017},
  organization={IEEE}
}
@article{pehle2023event,
  title={Event-based Backpropagation for Analog Neuromorphic Hardware},
  author={Pehle, Christian and Blessing, Luca and Arnold, Elias and M{\"u}ller, Eric and Schemmel, Johannes},
  journal={arXiv preprint arXiv:2302.07141},
  year={2023}
}


@ARTICLE{Davies18loihi,
  author={Davies, Mike and Srinivasa, Narayan and Lin, Tsung-Han and Chinya, Gautham and Cao, Yongqiang and Choday, Sri Harsha and Dimou, Georgios and Joshi, Prasad and Imam, Nabil and Jain, Shweta and Liao, Yuyun and Lin, Chit-Kwan and Lines, Andrew and Liu, Ruokun and Mathaikutty, Deepak and McCoy, Steven and Paul, Arnab and Tse, Jonathan and Venkataramanan, Guruguhanathan and Weng, Yi-Hsin and Wild, Andreas and Yang, Yoonseok and Wang, Hong},
  journal={IEEE Micro}, 
  title={Loihi: A Neuromorphic Manycore Processor with On-Chip Learning}, 
  year={2018},
  volume={38},
  number={1},
  pages={82-99},
  doi={10.1109/MM.2018.112130359}}

@misc{loihi2techbrief,
  title = {Taking Neuromorphic Computing to the Next Level with Loihi 2},
  howpublished= {\url{https://www.intel.com/content/www/us/en/research/neuromorphic-computing-loihi-2-technology-brief.html}},
  author={Intel},
  year = {2021},
}

@misc{mayr2019spinnaker,
      title={SpiNNaker 2: A 10 Million Core Processor System for Brain Simulation and Machine Learning}, 
      author={Christian Mayr and Sebastian Hoeppner and Steve Furber},
      year={2019},
      eprint={1911.02385},
      archivePrefix={arXiv},
      primaryClass={cs.ET}
}

@ARTICLE{painkras13spinnaker,
  author={Painkras, Eustace and Plana, Luis A. and Garside, Jim and Temple, Steve and Galluppi, Francesco and Patterson, Cameron and Lester, David R. and Brown, Andrew D. and Furber, Steve B.},
  journal={IEEE Journal of Solid-State Circuits}, 
  title={SpiNNaker: A 1-W 18-Core System-on-Chip for Massively-Parallel Neural Network Simulation}, 
  year={2013},
  volume={48},
  number={8},
  pages={1943-1953},
  doi={10.1109/JSSC.2013.2259038}}

@misc{pehle2022brainscales2,
      title={The BrainScaleS-2 accelerated neuromorphic system with hybrid plasticity}, 
      author={Christian Pehle and Sebastian Billaudelle and Benjamin Cramer and Jakob Kaiser and Korbinian Schreiber and Yannik Stradmann and Johannes Weis and Aron Leibfried and Eric Müller and Johannes Schemmel},
      year={2022},
      eprint={2201.11063},
      archivePrefix={arXiv},
      primaryClass={cs.NE}
}

@article{Kirkpatrick2017,
author = {James Kirkpatrick  and Razvan Pascanu  and Neil Rabinowitz  and Joel Veness  and Guillaume Desjardins  and Andrei A. Rusu  and Kieran Milan  and John Quan  and Tiago Ramalho  and Agnieszka Grabska-Barwinska  and Demis Hassabis  and Claudia Clopath  and Dharshan Kumaran  and Raia Hadsell },
title = {Overcoming catastrophic forgetting in neural networks},
journal = {Proceedings of the National Academy of Sciences},
volume = {114},
number = {13},
pages = {3521-3526},
year = {2017},
doi = {10.1073/pnas.1611835114},
URL = {https://www.pnas.org/doi/abs/10.1073/pnas.1611835114},
eprint = {https://www.pnas.org/doi/pdf/10.1073/pnas.1611835114},
}

﻿@Article{vandeVen2020,
author={van de Ven, Gido M. and Siegelmann, Hava T. and Tolias, Andreas S.}, 
title={Brain-inspired replay for continual learning with artificial neural networks},
journal={Nature Communications},
year={2020},
month={Aug},
day={13},
volume={11},
number={1},
pages={4069},
issn={2041-1723},
doi={10.1038/s41467-020-17866-2},
url={https://doi.org/10.1038/s41467-020-17866-2}
}

﻿@Article{Smith2022,
author={Smith, J. Darby and Hill, Aaron J. and Reeder, Leah E. and Franke, Brian C. and Lehoucq, Richard B. and Parekh, Ojas and Severa, William and Aimone, James B.},
title={Neuromorphic scaling advantages for energy-efficient random walk computations},
journal={Nature Electronics},
year={2022},
month={Feb},
day={01},
volume={5},
number={2},
pages={102-112},
issn={2520-1131},
doi={10.1038/s41928-021-00705-7},
url={https://doi.org/10.1038/s41928-021-00705-7}
}

@misc{Herridge2022, 
author = {Linda Herridge}, 
title = {NASA Satellites Launch Aboard Virgin Orbit’s LauncherOne}, 
year = 2022, 
url = {https://blogs.nasa.gov/kennedy/tag/ames-research-center/}, 
urldate = {2023-03-19}
}

@misc{Ward2022, 
author = {Sally Ward-Foxton}, 
title = {Mercedes Applies Neuromorphic Computing in EV Concept Car}, 
year = 2022, 
url = {https://www.eetimes.com/mercedes-applies-neuromorphic-computing-in-ev-concept-car/}, 
urldate = {2023-03-19}
}


@ARTICLE{Wu2022,
  title    = "Brain-inspired global-local learning incorporated with neuromorphic computing",
  author   = "Wu, Yujie and Zhao, Rong and Zhu, Jun and Chen, Feng and Xu, Mingkun and Li, Guoqi and Song, Sen and Deng, Lei and Wang, Guanrui and Zheng, Hao and Ma, Songchen and Pei, Jing and Zhang, Youhui and Zhao, Mingguo and Shi, Luping",
  journal  = "Nature Communications",
  volume   =  13,
  number   =  1,
  pages    = "65",
  month    =  jan,
  year     =  2022
}

@ARTICLE{NeuromorphicElasticControl2016,
AUTHOR={Stratmann, Philipp and Lakatos, Dominic and Albu-Schäffer, Alin},   
TITLE={Neuromodulation and Synaptic Plasticity for the Control of Fast Periodic Movement: Energy Efficiency in Coupled Compliant Joints via PCA},      
JOURNAL={Frontiers in Neurorobotics},      
VOLUME={10},           
YEAR={2016},      
URL={https://www.frontiersin.org/articles/10.3389/fnbot.2016.00002},       
DOI={10.3389/fnbot.2016.00002},      
ISSN={1662-5218},   
}

@ARTICLE{thorpe-2001,
AUTHOR={S Thorpe and A Delorme and R Van Rullen},   
TITLE={Spike-based strategies for rapid processing},      
JOURNAL={Neural Networks},      
VOLUME={14},           
YEAR={2001},      
number={6-7}
}

@ARTICLE{Covi2021,
AUTHOR={Covi, Erika and Donati, Elisa and Liang, Xiangpeng and Kappel, David and Heidari, Hadi and Payvand, Melika and Wang, Wei},
TITLE={Adaptive Extreme Edge Computing for Wearable Devices},
JOURNAL={Frontiers in Neuroscience},
VOLUME={15},
YEAR={2021},
URL={https://www.frontiersin.org/articles/10.3389/fnins.2021.611300},
DOI={10.3389/fnins.2021.611300},
ISSN={1662-453X},   
}

@InProceedings{Spilger2020,
author="Spilger, Philipp and M{\"u}ller, Eric and Emmel, Arne and Leibfried, Aron and Mauch, Christian and Pehle, Christian and Weis, Johannes and Breitwieser, Oliver and Billaudelle, Sebastian and Schmitt, Sebastian and Wunderlich, Timo C. and Stradmann, Yannik and Schemmel, Johannes",
editor="Gama, Joao and Pashami, Sepideh and Bifet, Albert and Sayed-Mouchawe, Moamar and Fr{\"o}ning, Holger and Pernkopf, Franz and Schiele, Gregor and Blott, Michaela",
title="hxtorch: PyTorch for BrainScaleS-2",
booktitle="IoT Streams for Data-Driven Predictive Maintenance and IoT, Edge, and Mobile for Embedded Machine Learning",
year="2020",
publisher="Springer International Publishing",
address="Cham",
pages="189--200",
isbn="978-3-030-66770-2"
}

@INPROCEEDINGS{Guangzhi2019,
  author={Tang, Guangzhi and Shah, Arpit and Michmizos, Konstantinos P.},
  booktitle={2019 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)}, 
  title={Spiking Neural Network on Neuromorphic Hardware for Energy-Efficient Unidimensional SLAM}, 
  year={2019},
  volume={},
  number={},
  pages={4176-4181},
  doi={10.1109/IROS40897.2019.8967864}}

﻿@Article{Bartolozzi2022,
author={Bartolozzi, Chiara and Indiveri, Giacomo and Donati, Elisa},
title={Embodied neuromorphic intelligence},
journal={Nature Communications},
year={2022},
month={Feb},
day={23},
volume={13},
number={1},
pages={1024},
issn={2041-1723},
doi={10.1038/s41467-022-28487-2},
url={https://doi.org/10.1038/s41467-022-28487-2}
}

@article{Croon2022,
author = {G. C. H. E. de Croon  and J. J. G. Dupeyroux  and S. B. Fuller  and J. A. R. Marshall },
title = {Insect-inspired AI for autonomous robots},
journal = {Science Robotics},
volume = {7},
number = {67},
pages = {eabl6334},
year = {2022},
doi = {10.1126/scirobotics.abl6334},
URL = {https://www.science.org/doi/abs/10.1126/scirobotics.abl6334},
eprint = {https://www.science.org/doi/pdf/10.1126/scirobotics.abl6334},
}

@ARTICLE{Soures2019,
AUTHOR={Soures, Nicholas and Kudithipudi, Dhireesha},
TITLE={Deep Liquid State Machines With Neural Plasticity for Video Activity Recognition},
JOURNAL={Frontiers in Neuroscience},
VOLUME={13},
YEAR={2019},
URL={https://www.frontiersin.org/articles/10.3389/fnins.2019.00686},
DOI={10.3389/fnins.2019.00686},
ISSN={1662-453X},
}



@INPROCEEDINGS{Vitale2021,
  author={Vitale, Antonio and Renner, Alpha and Nauer, Celine and Scaramuzza, Davide and Sandamirskaya, Yulia},
  booktitle={IEEE International Conference on Robotics and Automation (ICRA)}, 
  title={Event-driven Vision and Control for UAVs on a Neuromorphic Chip}, 
  year={2021},
  volume={},
  number={},
  pages={103-109},
  doi={10.1109/ICRA48506.2021.9560881}}

@ARTICLE{Su2023,
  author={Su, Fei and Liu, Chunsheng and Stratigopoulos, Haralampos-G.},
  journal={IEEE Design \& Test}, 
  title={Testability and Dependability of AI Hardware: Survey, Trends, Challenges, and Perspectives}, 
  year={2023},
  volume={40},
  number={2},
  pages={8-58},
  doi={10.1109/MDAT.2023.3241116}}


@ARTICLE{Krestinskaya2020,
  author={Krestinskaya, Olga and James, Alex Pappachen and Chua, Leon Ong},
  journal={IEEE Transactions on Neural Networks and Learning Systems}, 
  title={Neuromemristive Circuits for Edge Computing: A Review}, 
  year={2020},
  volume={31},
  number={1},
  pages={4-23},
  doi={10.1109/TNNLS.2019.2899262}}


@ARTICLE{Stratmann2017,
  author={Stratmann, Philipp and Lakatos, Dominic and Özparpucu, Mehmet C. and Albu-Schäffer, Alin},
  journal={IEEE Robotics and Automation Letters}, 
  title={Legged Elastic Multibody Systems: Adjusting Limit Cycles to Close-to-Optimal Energy Efficiency}, 
  year={2017},
  volume={2},
  number={2},
  pages={436-443},
  doi={10.1109/LRA.2016.2633580}}



@ARTICLE{Schuman2022,
  title    = "Opportunities for neuromorphic computing algorithms and
              applications",
  author   = "Schuman, Catherine D and Kulkarni, Shruti R and Parsa, Maryam and
              Mitchell, J Parker and Date, Prasanna and Kay, Bill",
  journal  = "Nature Computational Science",
  volume   =  2,
  number   =  1,
  pages    = "10--19",
  month    =  jan,
  year     =  2022
}


@article{stuijt2021mubrain,
  title={$\mu$Brain: An event-driven and fully synthesizable architecture for spiking neural networks},
  author={Stuijt, Jan and Sifalakis, Manolis and Yousefzadeh, Amirreza and Corradi, Federico},
  journal={Frontiers in neuroscience},
  pages={538},
  year={2021},
  publisher={Frontiers}
}

@book{puaun1998dna,
  title={DNA computing: new computing paradigms},
  author={P{\u{a}}un, Gheorghe and Rozenberg, Grzegorz and Salomaa, Arto},
  year={1998},
  publisher={Springer}
}
 
@article{maass1997networks,
  title={Networks of spiking neurons: the third generation of neural network models},
  author={Maass, Wolfgang},
  journal={Neural networks},
  volume={10},
  number={9},
  pages={1659--1671},
  year={1997},
  publisher={Elsevier}
}
 
@article{wan2022compute,
  title={A compute-in-memory chip based on resistive random-access memory},
  author={Wan, Weier and Kubendran, Rajkumar and Schaefer, Clemens and Eryilmaz, Sukru Burc and Zhang, Wenqiang and Wu, Dabin and Deiss, Stephen and Raina, Priyanka and Qian, He and Gao, Bin and others},
  journal={Nature},
  volume={608},
  number={7923},
  pages={504--512},
  year={2022},
  publisher={Nature Publishing Group UK London}
}
 
@article{payvand2022self,
  title={Self-organization of an inhomogeneous memristive hardware for sequence learning},
  author={Payvand, Melika and Moro, Filippo and Nomura, Kumiko and Dalgaty, Thomas and Vianello, Elisa and Nishi, Yoshifumi and Indiveri, Giacomo},
  journal={Nature communications},
  volume={13},
  number={1},
  pages={5793},
  year={2022},
  publisher={Nature Publishing Group UK London}
}
 
@article{eshraghian2022memristor,
  title={Memristor-based binarized spiking neural networks: Challenges and applications},
  author={Eshraghian, Jason K and Wang, Xinxin and Lu, Wei D},
  journal={IEEE Nanotechnology Magazine},
  volume={16},
  number={2},
  pages={14--23},
  year={2022},
  publisher={IEEE}
}
 
@article{modaresi2023openspike,
  title={OpenSpike: An OpenRAM SNN Accelerator},
  author={Modaresi, Farhad and Guthaus, Matthew and Eshraghian, Jason K},
  journal={arXiv preprint arXiv:2302.01015},
  year={2023}
}
 


@article{he2022implantable,
  title={An Implantable Neuromorphic Sensing System Featuring Near-Sensor Computation and Send-on-Delta Transmission for Wireless Neural Sensing of Peripheral Nerves},
  author={He, Yuming and Corradi, Federico and Shi, Chengyao and van der Ven, Stan and Timmermans, Martijn and Stuijt, Jan and Detterer, Paul and Harpe, Pieter and Lindeboom, Lucas and Hermeling, Evelien and others},
  journal={IEEE Journal of Solid-State Circuits},
  volume={57},
  number={10},
  pages={3058--3070},
  year={2022},
  publisher={IEEE}
}


@article{mackey1977oscillation,
  title={Oscillation and chaos in physiological control systems},
  author={Mackey, Michael C and Glass, Leon},
  journal={Science},
  volume={197},
  number={4300},
  pages={287--289},
  year={1977},
  publisher={American Association for the Advancement of Science}
}
@article{atiya2000new,
  title={New results on recurrent network training: unifying the algorithms and accelerating convergence},
  author={Atiya, Amir F and Parlos, Alexander G},
  journal={IEEE transactions on neural networks},
  volume={11},
  number={3},
  pages={697--709},
  year={2000},
  publisher={IEEE}
}



@article{jaeger2004harnessing,
  title={Harnessing nonlinearity: Predicting chaotic systems and saving energy in wireless communication},
  author={Jaeger, Herbert and Haas, Harald},
  journal={science},
  volume={304},
  number={5667},
  pages={78--80},
  year={2004},
  publisher={American Association for the Advancement of Science}
}

@article{mukhopadhyay2020learning,
  title={Learning dynamical systems in noise using convolutional neural networks},
  author={Mukhopadhyay, Sumona and Banerjee, Santo},
  journal={Chaos: An Interdisciplinary Journal of Nonlinear Science},
  volume={30},
  number={10},
  pages={103125},
  year={2020},
  publisher={AIP Publishing LLC}
}
@article{hennessy2019new,
  title={A new golden age for computer architecture},
  author={Hennessy, John L and Patterson, David A},
  journal={Communications of the ACM},
  volume={62},
  number={2},
  pages={48--60},
  year={2019},
  publisher={ACM New York, NY, USA}
}



@inproceedings{chilkuri2021parallelizing,
  title={Parallelizing legendre memory unit training},
  author={Chilkuri, Narsimha Reddy and Eliasmith, Chris},
  booktitle={International Conference on Machine Learning},
  pages={1898--1907},
  year={2021},
  organization={PMLR}
}

@ARTICLE{Indiveri2011,
  
AUTHOR={Indiveri, Giacomo and Linares-Barranco, Bernabe and Hamilton, Tara and van Schaik, André and Etienne-Cummings, Ralph and Delbruck, Tobi and Liu, Shih-Chii and Dudek, Piotr and Häfliger, Philipp and Renaud, Sylvie and Schemmel, Johannes and Cauwenberghs, Gert and Arthur, John and Hynna, Kai and Folowosele, Fopefolu and SAÏGHI, Sylvain and Serrano-Gotarredona, Teresa and Wijekoon, Jayawan and Wang, Yingxue and Boahen, Kwabena},   
	 
TITLE={Neuromorphic Silicon Neuron Circuits},      
	
JOURNAL={Frontiers in Neuroscience},      
	
VOLUME={5},           
	
YEAR={2011},      
	  
URL={https://www.frontiersin.org/articles/10.3389/fnins.2011.00073},       
	
DOI={10.3389/fnins.2011.00073},      
	
ISSN={1662-453X},   
   
ABSTRACT={Hardware implementations of spiking neurons can be extremely useful for a large variety of applications, ranging from high-speed modeling of large-scale neural systems to real-time behaving systems, to bidirectional brain–machine interfaces. The specific circuit solutions used to implement silicon neurons depend on the application requirements. In this paper we describe the most common building blocks and techniques used to implement these circuits, and present an overview of a wide range of neuromorphic silicon neurons, which implement different computational models, ranging from biophysically realistic and conductance-based Hodgkin–Huxley models to bi-dimensional generalized adaptive integrate and fire models. We compare the different design methodologies used for each silicon neuron design described, and demonstrate their features with experimental results, measured from a wide range of fabricated VLSI chips.}
}

@article{Timcheck2023, abstract = {A critical enabler for progress in neuromorphic computing research is the ability to transparently evaluate different neuromorphic solutions on important tasks and to compare them to state-of-the-art conventional solutions. The Intel Neuromorphic Deep Noise Suppression Challenge (Intel N-DNS Challenge), inspired by the Microsoft DNS Challenge, tackles a ubiquitous and commercially relevant task: real-time audio denoising. Audio denoising is likely to reap the benefits of neuromorphic computing due to its low-bandwidth, temporal nature and its relevance for low-power devices. The Intel N-DNS Challenge consists of two tracks: a simulation-based algorithmic track to encourage algorithmic innovation, and a neuromorphic hardware (Loihi 2) track to rigorously evaluate solutions. For both tracks, we specify an evaluation methodology based on energy, latency, and resource consumption in addition to output audio quality. We make the Intel N-DNS Challenge dataset scripts and evaluation code freely accessible, encourage community participation with monetary prizes, and release a neuromorphic baseline solution which shows promising audio quality, high power efficiency, and low resource consumption when compared to Microsoft NsNet2 and a proprietary Intel denoising model used in production. We hope the Intel N-DNS Challenge will hasten innovation in neuromorphic algorithms research, especially in the area of training tools and methods for real-time signal processing. We expect the winners of the challenge will demonstrate that for problems like audio denoising, significant gains in power and resources can be realized on neuromorphic devices available today compared to conventional state-of-the-art solutions.}, author = {Jonathan Timcheck and Sumit Bam Shrestha and Daniel Ben Dayan Rubin and Adam Kupryjanow and Garrick Orchard and Lukasz Pindor and Timothy Shea and Mike Davies}, month = {3}, title = {The Intel Neuromorphic DNS Challenge}, url = {http://arxiv.org/abs/2303.09503}, year = {2023}, } 

@article{Peres2022, abstract = {Learning and development in real brains typically happens over long timescales, making long-term exploration of these features a significant research challenge. One way to address this problem is to use computational models to explore the brain, with Spiking Neural Networks a popular choice to capture neuron and synapse dynamics. However, researchers require simulation tools and platforms to execute simulations in real- or sub-realtime, to enable exploration of features such as long-term learning and neural pathologies over meaningful periods. This article presents novel multicore processing strategies on the SpiNNaker Neuromorphic hardware, addressing parallelization of Spiking Neural Network operations through allocation of dedicated computational units to specific tasks (such as neural and synaptic processing) to optimize performance. The work advances previous real-time simulations of a cortical microcircuit model, parameterizing load balancing between computational units in order to explore trade-offs between computational complexity and speed, to provide the best fit for a given application. By exploiting the flexibility of the SpiNNaker Neuromorphic platform, up to 9× throughput of neural operations is demonstrated when running biologically representative Spiking Neural Networks.}, author = {Luca Peres and Oliver Rhodes}, doi = {10.3389/fnins.2022.867027}, issn = {1662453X}, journal = {Frontiers in Neuroscience}, keywords = {SpiNNaker,event-driven simulation,neuromorphic computing,parallel programming,real-time,spiking neural networks}, month = {5}, publisher = {Frontiers Media S.A.}, title = {Parallelization of Neural Processing on Neuromorphic Hardware}, volume = {16}, year = {2022}, } 

@article{banbury2021mlperf,
  title={MLPerf Tiny Benchmark},
  author={Banbury, Colby and Reddi, Vijay Janapa and Torelli, Peter and Holleman, Jeremy and Jeffries, Nat and Kiraly, Csaba and Montino, Pietro and Kanter, David and Ahmed, Sebastian and Pau, Danilo and others},
  journal={Proceedings of the Neural Information Processing Systems Track on Datasets and Benchmarks},
  year={2021}
}
@article{Knight2021,
    author = {Knight, James C and Komissarov, Anton and Nowotny, Thomas},
    doi = {10.3389/fninf.2021.659005},
    issn = {1662-5196},
    journal = {Frontiers in Neuroinformatics},
    month = {apr},
    number = {April},
    title = {{PyGeNN: A Python Library for GPU-Enhanced Neural Networks}},
    url = {https://www.frontiersin.org/articles/10.3389/fninf.2021.659005/full},
    volume = {15},
    year = {2021}
}

@article{anumula2018feature,
  title={Feature representations for neuromorphic audio spike streams},
  author={Anumula, Jithendar and Neil, Daniel and Delbruck, Tobi and Liu, Shih-Chii},
  journal={Frontiers in neuroscience},
  volume={12},
  pages={23},
  year={2018},
  publisher={Frontiers Media SA}
}

@article{bohte2002error,
  title={Error-backpropagation in temporally encoded networks of spiking neurons},
  author={Bohte, Sander M and Kok, Joost N and La Poutre, Han},
  journal={Neurocomputing},
  volume={48},
  number={1-4},
  pages={17--37},
  year={2002},
  publisher={Elsevier}
}

@article{chan2007aer,
  title={{AER} {EAR}: A matched silicon cochlea pair with address event representation interface},
  author={Chan, Vincent and Liu, Shih-Chii and van Schaik, Andr},
  journal={IEEE Transactions on Circuits and Systems I: Regular Papers},
  volume={54},
  number={1},
  pages={48--59},
  year={2007},
  publisher={IEEE}
}

@article{gollisch2008rapid,
  title={Rapid neural coding in the retina with relative spike latencies},
  author={Gollisch, Tim and Meister, Markus},
  journal={science},
  volume={319},
  number={5866},
  pages={1108--1111},
  year={2008},
  publisher={American Association for the Advancement of Science}
}

@article{heeger2000poisson,
  title={Poisson model of spike generation},
  author={Heeger, David and others},
  journal={Handout, University of Standford},
  volume={5},
  number={1-13},
  pages={76},
  year={2000}
}

@Article{leonard1993tidigits,
  Title = {Tidigits speech corpus},
  Author = {Leonard, R Gary and Doddington, George},
  Journal = {Texas Instruments, Inc},
  Year = {1993}
}

@article{magnasco2003wave,
  title={A wave traveling over a Hopf instability shapes the cochlear tuning curve},
  author={Magnasco, Marcelo O},
  journal={Physical review letters},
  volume={90},
  number={5},
  pages={058101},
  year={2003},
  publisher={APS}
}

@article{mainen1995reliability,
  title={Reliability of spike timing in neocortical neurons},
  author={Mainen, Zachary F and Sejnowski, Terrence J},
  journal={Science},
  volume={268},
  number={5216},
  pages={1503--1506},
  year={1995},
  publisher={American Association for the Advancement of Science}
}

@article{pillow2005prediction,
  title={Prediction and decoding of retinal ganglion cell responses with a probabilistic spiking model},
  author={Pillow, Jonathan W and Paninski, Liam and Uzzell, Valerie J and Simoncelli, Eero P and Chichilnisky, EJ},
  journal={Journal of Neuroscience},
  volume={25},
  number={47},
  pages={11003--11013},
  year={2005},
  publisher={Soc Neuroscience}
}

@article{embodied_Turing,
  title={Catalyzing next-generation Artificial Intelligence through NeuroAI
},
  author={A. Zador and et. al.},
  journal={Nature Communications},
  volume={14},
  number={1597},
  year={2023}
}

@article{piee-review-2015,
  title={Memory and information processing in neuromorphic systems},
  author={G. Indiveri and S. C. Liu},
  journal={Proceedings of IEEE},
  volume={103},
  number={8},
  pages={1379-97},
  year={2015}
}

@article{pillow2008spatio,
  title={Spatio-temporal correlations and visual signalling in a complete neuronal population},
  author={Pillow, Jonathan W and Shlens, Jonathon and Paninski, Liam and Sher, Alexander and Litke, Alan M and Chichilnisky, EJ and Simoncelli, Eero P},
  journal={Nature},
  volume={454},
  number={7207},
  pages={995--999},
  year={2008},
  publisher={Nature Publishing Group UK London}
}

@article{serrano2005aer,
  title={{AER} building blocks for multi-layer multi-chip neuromorphic vision systems},
  author={Serrano-Gotarredona, Rafael and Oster, Matthias and Lichtsteiner, Patrick and Linares-Barranco, Alejandro and Paz-Vicente, Rafael and Gomez-Rodriguez, Francisco and Kolle Riis, H{\aa}vard and Delbruck, T and Liu, Shih-Chii and Zahnd, Sam and others},
  journal={Advances in neural information processing systems},
  volume={18},
  year={2005}
}

@article{shrestha2018slayer,
  title={{SLAYER}: Spike layer error reassignment in time},
  author={Shrestha, Sumit B and Orchard, Garrick},
  journal={Advances in neural information processing systems},
  volume={31},
  year={2018}
}

@inproceedings{shrestha2022spikemax,
  title={Spikemax: Spike-based Loss Methods for Classification},
  author={Shrestha, Sumit Bam and Zhu, Longwei and Sun, Pengfei},
  booktitle={2022 International Joint Conference on Neural Networks (IJCNN)},
  pages={1--7},
  year={2022},
  organization={IEEE}
}

@article{van2001rate,
  title={Rate coding versus temporal order coding: what the retinal ganglion cells tell the visual cortex},
  author={Van Rullen, Rufin and Thorpe, Simon J},
  journal={Neural computation},
  volume={13},
  number={6},
  pages={1255--1283},
  year={2001},
  publisher={MIT Press}
}

@article{zilany2014updated,
  title={Updated parameters and expanded simulation options for a model of the auditory periphery},
  author={Zilany, Muhammad SA and Bruce, Ian C and Carney, Laurel H},
  journal={The Journal of the Acoustical Society of America},
  volume={135},
  number={1},
  pages={283--286},
  year={2014},
  publisher={Acoustical Society of America}
}

@inproceedings{yousefzadeh2022seneca,
  title={SENeCA: Scalable energy-efficient neuromorphic computer architecture},
  author={Yousefzadeh, Amirreza and Van Schaik, Gert-Jan and Tahghighi, Mohammad and Detterer, Paul and Traferro, Stefano and Hijdra, Martijn and Stuijt, Jan and Corradi, Federico and Sifalakis, Manolis and Konijnenburg, Mario},
  booktitle={2022 IEEE 4th International Conference on Artificial Intelligence Circuits and Systems (AICAS)},
  pages={371--374},
  year={2022},
  organization={IEEE}
}



@inproceedings{tang2023seneca,
  title={Open the box of digital neuromorphic processor: Towards effective algorithm-hardware co-design},
  author={Tang, Guangzhi and Safa, Ali and Shidqi, Kevin and Detterer, Paul and Traferro, Stefano and Konijnenburg, Mario and Sifalakis, Manolis and van Schaik, Gert-Jan and Yousefzadeh, Amirreza},
  booktitle={2023 IEEE International Symposium on Circuits and Systems (ISCAS)},
  pages={1-5},
  year={2023},
  organization={IEEE}
}



@article{Yavuz2016,
    title = {{GeNN}: a code generation framework for accelerated brain simulations},
    volume = {6},
    issn = {2045-2322},
    url = {http://www.pubmedcentral.nih.gov/articlerender.fcgi?artid=4703976&tool=pmcentrez&rendertype=abstract},
    doi = {10.1038/srep18854},
    abstract = {Large-scale numerical simulations of detailed brain circuit models are important for identifying hypotheses on brain functions and testing their consistency and plausibility. An ongoing challenge for simulating realistic models is, however, computational speed. In this paper, we present the GeNN (GPU-enhanced Neuronal Networks) framework, which aims to facilitate the use of graphics accelerators for computational models of large-scale neuronal networks to address this challenge. GeNN is an open source library that generates code to accelerate the execution of network simulations on NVIDIA GPUs, through a flexible and extensible interface, which does not require in-depth technical knowledge from the users. We present performance benchmarks showing that 200-fold speedup compared to a single core of a CPU can be achieved for a network of one million conductance based Hodgkin-Huxley neurons but that for other models the speedup can differ. GeNN is available for Linux, Mac OS X and Windows platforms. The source code, user manual, tutorials, Wiki, in-depth example projects and all other related information can be found on the project website http://genn-team.github.io/genn/.},
    number = {1},
    journal = {Scientific Reports},
    author = {Yavuz, Esin and Turner, James and Nowotny, Thomas},
    month = may,
    year = {2016},
    pmid = {26740369},
    note = {Publisher: Nature Publishing Group},
    pages = {18854},
    file = {Yavuz et al_2016_GeNN.pdf:/its/home/jk421/zotero_gdrive/Yavuz et al_2016_GeNN.pdf:application/pdf},
}


@inproceedings{vineyard2019benchmarking,
  title={Benchmarking event-driven neuromorphic architectures},
  author={Vineyard, Craig M and Green, Sam and Severa, William M and Ko{\c{c}}, {\c{C}}etin Kaya},
  booktitle={Proceedings of the International Conference on Neuromorphic Systems},
  pages={1--5},
  year={2019}
}

@INPROCEEDINGS{Orchard2021,
  author={Orchard, Garrick and Frady, E. Paxon and Rubin, Daniel Ben Dayan and Sanborn, Sophia and Shrestha, Sumit Bam and Sommer, Friedrich T. and Davies, Mike},
  booktitle={2021 IEEE Workshop on Signal Processing Systems (SiPS)}, 
  title={Efficient Neuromorphic Signal Processing with Loihi 2}, 
  year={2021},
  volume={},
  number={},
  pages={254-259},
  doi={10.1109/SiPS52927.2021.00053}}


@article{davies2019benchmarks,
  title={Benchmarks for progress in neuromorphic computing},
  author={Davies, Mike},
  journal={Nature Machine Intelligence},
  volume={1},
  number={9},
  pages={386--388},
  year={2019},
  publisher={Nature Publishing Group}
}

@article{jetcas-review-basu,
  title={Low-power, adaptive neuromorphic systems: Recent progress and future directions},
  author={A. Basu and J. Acharya and T. Karnik and H. Liu and et. al.},
  journal={IEEE Journal on Emerging and Selected Topics in Circuits and Systems},
  volume={8},
  number={1},
  pages={6-27},
  year={2018},
}

@inproceedings{dubey2022icassp,
  title={ICASSP 2022 Deep Noise Suppression Challenge},
  author={Dubey, Harishchandra and Gopal, Vishak and Cutler, Ross and Matusevych, Sergiy and Braun, Sebastian and Eskimez, Emre Sefik and Thakker, Manthan and Yoshioka, Takuya and Gamper, Hannes and Aichner, Robert},
  booktitle={ICASSP},
  year={2022}
}

@inproceedings{cicc-review-basu,
  title={Spiking neural network integrated circuits: A review of trends and future directions},
  author={A. Basu and L. Deng and C. Frenkel and X. Zhang},
  booktitle={IEEE Custom Integrated Circuits Conference (CICC)},
  year={2022}
}

@article{ceolini2020hand,
  title={Hand-gesture recognition based on EMG and event-based camera sensor fusion: A benchmark in neuromorphic computing},
  author={Ceolini, Enea and Frenkel, Charlotte and Shrestha, Sumit Bam and Taverni, Gemma and Khacef, Lyes and Payvand, Melika and Donati, Elisa},
  journal={Frontiers in Neuroscience},
  pages={637},
  year={2020},
  publisher={Frontiers}
}

@article{davies2021advancing,
  title={Advancing neuromorphic computing with Loihi: A survey of results and outlook},
  author={Davies, Mike and Wild, Andreas and Orchard, Garrick and Sandamirskaya, Yulia and Guerra, Gabriel A Fonseca and Joshi, Prasad and Plank, Philipp and Risbud, Sumedh R},
  journal={Proceedings of the IEEE},
  volume={109},
  number={5},
  pages={911--934},
  year={2021},
  publisher={IEEE}
}
 
@article{liu2018memory,
  title={Memory-efficient deep learning on a SpiNNaker 2 prototype},
  author={Liu, Chen and Bellec, Guillaume and Vogginger, Bernhard and Kappel, David and Partzsch, Johannes and Neum{\"a}rker, Felix and H{\"o}ppner, Sebastian and Maass, Wolfgang and Furber, Steve B and Legenstein, Robert and others},
  journal={Frontiers in neuroscience},
  volume={12},
  pages={840},
  year={2018},
  publisher={Frontiers Media SA}
}

@article{ccakal2023training,
  title={Training and Deploying Spiking NN Applications to the Mixed-Signal Neuromorphic Chip Dynap-SE2 with Rockpool},
  author={{\c{C}}akal, U{\u{g}}urcan and Ulusoy, Ilkay and Muir, Dylan R},
  journal={arXiv preprint arXiv:2303.12167},
  year={2023}
}

@article{goltz2021fast,
  title={Fast and energy-efficient neuromorphic deep learning with first-spike times},
  author={G{\"o}ltz, Julian and Kriener, Laura and Baumbach, Andreas and Billaudelle, Sebastian and Breitwieser, Oliver and Cramer, Benjamin and Dold, Dominik and Kungl, Akos Ferenc and Senn, Walter and Schemmel, Johannes and others},
  journal={Nature machine intelligence},
  volume={3},
  number={9},
  pages={823--835},
  year={2021},
  publisher={Nature Publishing Group UK London}
}

@article{sharifshazileh2021electronic,
  title={An electronic neuromorphic system for real-time detection of high frequency oscillations (HFO) in intracranial EEG},
  author={Sharifshazileh, Mohammadali and Burelo, Karla and Sarnthein, Johannes and Indiveri, Giacomo},
  journal={Nature communications},
  volume={12},
  number={1},
  pages={3095},
  year={2021},
  publisher={Nature Publishing Group UK London}
}


@article{laborieux2021synaptic,
  title={Synaptic metaplasticity in binarized neural networks},
  author={Laborieux, Axel and Ernoult, Maxence and Hirtzlin, Tifenn and Querlioz, Damien},
  journal={Nature communications},
  volume={12},
  number={1},
  pages={2549},
  year={2021},
  publisher={Nature Publishing Group UK London}
}



 
@incollection{turing1948,
    author = {Turing, Alan},
    isbn = {9780198250791},
    title = "{395Intelligent Machinery (1948)}",
    booktitle = "{The Essential Turing}",
    publisher = {Oxford University Press},
    year = {2004},
    month = {09},
    abstract = "{By the beginning of 1947 much effort had gone into writing programmes or â€˜instruction tablesâ€™ for the ACE. In â€˜Proposed Electronic Calculatorâ€™, Turing had said that work on instruction tables should start immediately, since the â€˜earlier stages of the making of instruction tables will have serious repercussions on the design [of the machine]â€™; moreover, the programming work should â€˜go on whilst the machine is being built, in order to avoid some of the delay between the delivery of the machine and the production of resultsâ€™. However, little progress had been made on the physical construction of the ACE. The actual engineering work was being carried out not at the National Physical Laboratory but at the Post Office Research Station, under the supervision of Turingâ€™s wartime associate Flowers (see the introductions to Chapters 4 and 9). Flowers was asked by the NPL early in 1946 to assist with the engineering design of, and to build, the ACE. Ominously, the letter of agreement from Flowersâ€™s superior to Turingâ€™s superior spoke of â€˜very considerable arrears of workâ€™ and warned that â€˜the manpower position is difficultâ€™. Initial progress was nevertheless promising, with some early successes in the experimental work on the delay line memory units. According to an NPL document dated March 1946, â€˜Mr. Flowers states that they can have ready for N.P.L. a minimal ACE by August or September.â€™ Unfortunately it proved impossible to keep to Flowersâ€™s timetable. Dollis Hill was occupied with a backlog of urgent work on the national telephone system (at that time managed by the Post Office). Flowersâ€™s Section was â€˜too busy to do other peopleâ€™s workâ€™ (he said in 1998). Only two men could be spared to work on the ACE, Chandler and Coombs (both of whom had played leading roles in the wartime Colossus project). Sir Charles Darwin, the Director of the NPL, noted in August 1946 that the Post Office was â€˜not in a position to plunge very deepâ€™, and by November was expressing concern to Post Office staff about the slow rate of progress on the ACE. The fault was not all with the Post Office, however.}",
    doi = {10.1093/oso/9780198250791.003.0016},
    url = {https://doi.org/10.1093/oso/9780198250791.003.0016},
    eprint = {https://academic.oup.com/book/0/chapter/355746030/chapter-pdf/43817005/isbn-9780198250791-book-part-16.pdf},
}

@book{eliasmith2003neural,
 IDS = {Eliasmith2003, eliasmith_2003},
 author = {Eliasmith, C  and Anderson, C  H },
 publisher = {{MIT} Press},
 title = {Neural Engineering: Computation, Representation, and Dynamics in Neurobiological Systems},
 year = {2003}
}


@article{kleyko2022vector,
  title={Vector symbolic architectures as a computing framework for emerging hardware},
  author={Kleyko, Denis and Davies, Mike and Frady, Edward Paxon and Kanerva, Pentti and Kent, Spencer J and Olshausen, Bruno A and Osipov, Evgeny and Rabaey, Jan M and Rachkovskij, Dmitri A and Rahimi, Abbas and others},
  journal={Proceedings of the IEEE},
  volume={110},
  number={10},
  pages={1538--1571},
  year={2022},
  publisher={IEEE}
}



@incollection{neumann51automata,
  added-at = {2010-10-07T11:09:10.000+0200},
  author = {von Neumann, J.},
  biburl = {https://www.bibsonomy.org/bibtex/2694ad7fd1d0653fb2b139aac4338535f/msn},
  booktitle = {Cerebral Mechanisms in Behaviour},
  description = {http://www.hfr.org.uk/cybernetics-pages/bibcyb-usymp.htm},
  editor = {Jeffress, L. A.},
  interhash = {041cc800acb9462705a4d54a7cc08bad},
  intrahash = {694ad7fd1d0653fb2b139aac4338535f},
  keywords = {cites.ref state.unclassified},
  publisher = {Wiley},
  timestamp = {2010-10-07T11:09:10.000+0200},
  title = {The general and logical theory of automata},
  year = 1951
}

@article{ILSVRC15,
Author = {Olga Russakovsky and Jia Deng and Hao Su and Jonathan Krause and Sanjeev Satheesh and Sean Ma and Zhiheng Huang and Andrej Karpathy and Aditya Khosla and Michael Bernstein and Alexander C. Berg and Li Fei-Fei},
Title = {{ImageNet Large Scale Visual Recognition Challenge}},
Year = {2015},
journal   = {International Journal of Computer Vision (IJCV)},
doi = {10.1007/s11263-015-0816-y},
volume={115},
number={3},
pages={211-252}
}

@article{brink2012learning,
  title={A learning-enabled neuron array IC based upon transistor channel models of biological phenomena},
  author={Brink, Stephen and Nease, Stephen and Hasler, Paul and Ramakrishnan, Shubha and Wunderlich, Richard and Basu, Arindam and Degnan, Brian},
  journal={IEEE Transactions on Biomedical Circuits and Systems},
  volume={7},
  number={1},
  pages={71--81},
  year={2012},
  publisher={IEEE}
}

@article{narma,
  title={Minimum complexity echo state network},
  author={A. Rodan and P. Tino},
  journal={IEEE Transactions on Neural Networks},
  volume={22},
  number={1},
  pages={131-144},
  year={2011},
  publisher={IEEE}
}

@article{ramakrishnan2013neuron,
  title={Neuron array with plastic synapses and programmable dendrites},
  author={Ramakrishnan, Shubha and Wunderlich, Richard and Hasler, Jennifer and George, Suma},
  journal={IEEE Transactions on biomedical circuits and systems},
  volume={7},
  number={5},
  pages={631--642},
  year={2013},
  publisher={IEEE}
}

@article{basu2010neural,
  title={Neural dynamics in reconfigurable silicon},
  author={Basu, Arindam and Ramakrishnan, Shubha and Petre, Csaba and Koziol, Scott and Brink, Stephen and Hasler, Paul E},
  journal={IEEE Transactions on Biomedical Circuits and Systems},
  volume={4},
  number={5},
  pages={311--319},
  year={2010},
  publisher={IEEE}
}
@Article{Chicca_etal14,
author		= {E. Chicca and F. Stefanini and C. Bartolozzi and G.
		  Indiveri},
title		= {Neuromorphic electronic circuits for building autonomous
		  cognitive systems},
journal		= {Proceedings of the {IEEE}},
year		= {2014},
month		= sep,
volume		= {102},
number		= {9},
pages		= {1367--1388},
keywords	= {Buildings;Computational modeling;Computer
		  architecture;Integrated circuit
		  modeling;Neuromorphics;Neurons;Cognitive systems;learning
		  systems;neuromorphic engineering;real-time neuromorphic
		  systems;spike-timing-dependent plasticity (STDP);spiking
		  neural network architecture;subthreshold analog
		  circuits;very large-scale integration
		  (VLSI);winner-take-all ({WTA})},
issn		= {0018-9219},
doi		= {10.1109/JPROC.2014.2313954}
}

@article{spilger2022hxtorch,
  title={hxtorch. snn: Machine-learning-inspired Spiking Neural Network Modeling on BrainScaleS-2},
  author={Spilger, Philipp and Arnold, Elias and Blessing, Luca and Mauch, Christian and Pehle, Christian and M{\"u}ller, Eric and Schemmel, Johannes},
  journal={arXiv preprint arXiv:2212.12210},
  year={2022}
}


@inproceedings{esmanhotto2020high,
  title={High-density 3D monolithically integrated multiple 1T1R multi-level-cell for neural networks},
  author={Esmanhotto, E and Brunet, L and Castellani, N and Bonnet, D and Dalgaty, T and Grenouillet, L and Ly, DRB and Cagli, C and Vizioz, C and Allouti, N and others},
  booktitle={2020 IEEE International Electron Devices Meeting (IEDM)},
  pages={36--5},
  year={2020},
  organization={IEEE}
}

@article{sebastian2020memory,
  title={Memory devices and applications for in-memory computing},
  author={Sebastian, Abu and Le Gallo, Manuel and Khaddam-Aljameh, Riduan and Eleftheriou, Evangelos},
  journal={Nature nanotechnology},
  volume={15},
  number={7},
  pages={529--544},
  year={2020},
  publisher={Nature Publishing Group UK London}
}
 
@article{boybat2018neuromorphic,
  title={Neuromorphic computing with multi-memristive synapses},
  author={Boybat, Irem and Le Gallo, Manuel and Nandakumar, SR and Moraitis, Timoleon and Parnell, Thomas and Tuma, Tomas and Rajendran, Bipin and Leblebici, Yusuf and Sebastian, Abu and Eleftheriou, Evangelos},
  journal={Nature communications},
  volume={9},
  number={1},
  pages={2514},
  year={2018},
  publisher={Nature Publishing Group UK London}
}

@inproceedings{mulaosmanovic2017novel,
  title={Novel ferroelectric FET based synapse for neuromorphic systems},
  author={Mulaosmanovic, H and Ocker, J and M{\"u}ller, S and Noack, M and M{\"u}ller, J and Polakowski, P and Mikolajick, T and Slesazeck, S},
  booktitle={2017 Symposium on VLSI Technology},
  pages={T176--T177},
  year={2017},
  organization={IEEE}
}

@article{vincent2015spin,
  title={Spin-transfer torque magnetic memory as a stochastic memristive synapse for neuromorphic systems},
  author={Vincent, Adrien F and Larroque, J{\'e}r{\^o}me and Locatelli, Nicolas and Romdhane, Nesrine Ben and Bichler, Olivier and Gamrat, Christian and Zhao, Wei Sheng and Klein, Jacques-Olivier and Galdin-Retailleau, Sylvie and Querlioz, Damien},
  journal={IEEE transactions on biomedical circuits and systems},
  volume={9},
  number={2},
  pages={166--174},
  year={2015},
  publisher={IEEE}
}
 
@article{torrejon2017neuromorphic,
  title={Neuromorphic computing with nanoscale spintronic oscillators},
  author={Torrejon, Jacob and Riou, Mathieu and Araujo, Flavio Abreu and Tsunegi, Sumito and Khalsa, Guru and Querlioz, Damien and Bortolotti, Paolo and Cros, Vincent and Yakushiji, Kay and Fukushima, Akio and others},
  journal={Nature},
  volume={547},
  number={7664},
  pages={428--431},
  year={2017},
  publisher={Nature Publishing Group UK London}
}

@article{shastri2021photonics,
  title={Photonics for artificial intelligence and neuromorphic computing},
  author={Shastri, Bhavin J and Tait, Alexander N and Ferreira de Lima, Thomas and Pernice, Wolfram HP and Bhaskaran, Harish and Wright, C David and Prucnal, Paul R},
  journal={Nature Photonics},
  volume={15},
  number={2},
  pages={102--114},
  year={2021},
  publisher={Nature Publishing Group UK London}
}



@inproceedings{yu_etal2020_IMCreview,
  title={Compute-in-memory with emerging nonvolatile-memories: challenges and prospects},
  author={Yu, Shimeng and Sun, Xiaoyu and Peng, Xiaochen and Huang, Shanshi},
  booktitle={2020 IEEE Custom Integrated Circuits Conference (CICC)},
  pages={1--4},
  year={2020},
  organization={IEEE}
}

@article{khaddam2022hermes,
  title={HERMES-core—A 1.59-TOPS/mm 2 PCM on 14-nm CMOS in-memory compute core using 300-ps/LSB linearized CCO-based ADCs},
  author={Khaddam-Aljameh, Riduan and Stanisavljevic, Milos and Mas, Jordi Fornt and Karunaratne, Geethan and Br{\"a}ndli, Matthias and Liu, Feng and Singh, Abhairaj and M{\"u}ller, Silvia M and Egger, Urs and Petropoulos, Anastasios and others},
  journal={IEEE Journal of Solid-State Circuits},
  volume={57},
  number={4},
  pages={1027--1038},
  year={2022},
  publisher={IEEE}
}


@inproceedings{valentian2019fully,
  title={Fully integrated spiking neural network with analog neurons and RRAM synapses},
  author={Valentian, A and Rummens, F and Vianello, E and Mesquida, T and de Boissac, C Lecat-Mathieu and Bichler, O and Reita, C},
  booktitle={2019 IEEE International Electron Devices Meeting (IEDM)},
  pages={14--3},
  year={2019},
  organization={IEEE}
}

@article{sebastian_etal2020_IMCreview,
  title={Memory devices and applications for in-memory computing},
  author={Sebastian, Abu and Le Gallo, Manuel and Khaddam-Aljameh, Riduan and Eleftheriou, Evangelos},
  journal={Nature nanotechnology},
  volume={15},
  number={7},
  pages={529--544},
  year={2020},
  publisher={Nature Publishing Group}
}

@article{payvand2019neuromorphic,
  title={A neuromorphic systems approach to in-memory computing with non-ideal memristive devices: From mitigation to exploitation},
  author={Payvand, Melika and Nair, Manu V and M{\"u}ller, Lorenz K and Indiveri, Giacomo},
  journal={Faraday Discussions},
  volume={213},
  pages={487--510},
  year={2019},
  publisher={Royal Society of Chemistry}
}

@inproceedings{demiraug2021pcm,
  title={PCM-trace: scalable synaptic eligibility traces with resistivity drift of phase-change materials},
  author={Demira{\u{g}}, Yi{\u{g}}it and Moro, Filippo and Dalgaty, Thomas and Navarro, Gabriele and Frenkel, Charlotte and Indiveri, Giacomo and Vianello, Elisa and Payvand, Melika},
  booktitle={2021 IEEE International Symposium on Circuits and Systems (ISCAS)},
  pages={1--5},
  year={2021},
  organization={IEEE}
}

@inproceedings{aimone2019composing,
  title={Composing neural algorithms with Fugu},
  author={Aimone, James B and Severa, William and Vineyard, Craig M},
  booktitle={Proceedings of the International Conference on Neuromorphic Systems},
  pages={1--8},
  year={2019}
}

@inproceedings{vineyard2022neural,
  title={Neural Mini-Apps as a Tool for Neuromorphic Computing Insight},
  author={Vineyard, Craig and Cardwell, Suma and Chance, Frances and Musuvathy, Srideep and Rothganger, Fred and Severa, William and Smith, John and Teeter, Corinne and Wang, Felix and Aimone, James},
  booktitle={Neuro-Inspired Computational Elements Conference},
  pages={40--49},
  year={2022}
}

@article{rothganger2014n2a,
  title={N2A: a computational tool for modeling from neurons to algorithms},
  author={Rothganger, Fredrick and Warrender, Christina E and Trumbo, Derek and Aimone, James B},
  journal={Frontiers in neural circuits},
  volume={8},
  pages={1},
  year={2014},
  publisher={Frontiers Media SA}
}

@misc{bai2019onnx,
    author = {Bai, Junjie and Lu, Fang and Zhang, Ke and others},
    title = {ONNX: Open Neural Network Exchange},
    year = {2019},
    publisher = {GitHub},
    journal = {GitHub repository},
    howpublished = {\url{https://github.com/onnx/onnx}},
    commit = {94d238d96e3fb3a7ba34f03c284b9ad3516163be}
}

@misc{chen2018tvm,
      title={TVM: An Automated End-to-End Optimizing Compiler for Deep Learning}, 
      author={Tianqi Chen and Thierry Moreau and Ziheng Jiang and Lianmin Zheng and Eddie Yan and Meghan Cowan and Haichen Shen and Leyuan Wang and Yuwei Hu and Luis Ceze and Carlos Guestrin and Arvind Krishnamurthy},
      year={2018},
      eprint={1802.04799},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@article{peng2020dnn+,
  title={DNN+ NeuroSim V2.0: An end-to-end benchmarking framework for compute-in-memory accelerators for on-chip training},
  author={Peng, Xiaochen and Huang, Shanshi and Jiang, Hongwu and Lu, Anni and Yu, Shimeng},
  journal={IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems},
  volume={40},
  number={11},
  pages={2306--2319},
  year={2020},
  publisher={IEEE}
}

@article{qiao2015reconfigurable,
  title={A reconfigurable on-line learning spiking neuromorphic processor comprising 256 neurons and 128K synapses},
  author={Qiao, Ning and Mostafa, Hesham and Corradi, Federico and Osswald, Marc and Stefanini, Fabio and Sumislawska, Dora and Indiveri, Giacomo},
  journal={Frontiers in neuroscience},
  volume={9},
  pages={141},
  year={2015},
  publisher={Frontiers Media SA}
}

@article{neckar2018braindrop,
  title={Braindrop: A mixed-signal neuromorphic architecture with a dynamical systems-based programming model},
  author={Neckar, Alexander and Fok, Sam and Benjamin, Ben V and Stewart, Terrence C and Oza, Nick N and Voelker, Aaron R and Eliasmith, Chris and Manohar, Rajit and Boahen, Kwabena},
  journal={Proceedings of the IEEE},
  volume={107},
  number={1},
  pages={144--164},
  year={2018},
  publisher={IEEE}
}


@article{xiao2022rainbow,
  title={Rainbow keywords: Efficient incremental learning for online spoken keyword spotting},
  author={Xiao, Yang and Hou, Nana and Chng, Eng Siong},
  journal={arXiv preprint arXiv:2203.16361},
  year={2022}
}


@inproceedings{huang2022progressive,
  title={Progressive continual learning for spoken keyword spotting},
  author={Huang, Yizheng and Hou, Nana and Chen, Nancy F},
  booktitle={ICASSP 2022-2022 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={7552--7556},
  year={2022},
  organization={IEEE}
}

@inproceedings{yin2022attentive,
  title={Attentive decision-making and dynamic resetting of continual running SRNNs for end-to-end streaming keyword spotting},
  author={Yin, Bojian and Guo, Qinghai and Corradi, Federico and Bohte, Sander},
  booktitle={Proceedings of the International Conference on Neuromorphic Systems 2022},
  pages={1--8},
  year={2022}
}


@inproceedings{tacos2021,
  title={TACOS: Task Agnostic Continual Learning in Spiking Neural Networks},
  author={Soures, Nicholas and Helfer, Peter and Daram, Anurag and Pandit, Tej and Kudithipudi, Dhireesha},
  booktitle={Theory and Foundation of Continual Learning Workshop at ICML’2021},
  year={July 2021}
}

@article{awasthi2021teaching,
  title={Teaching keyword spotters to spot new keywords with limited examples},
  author={Awasthi, Abhijeet and Kilgour, Kevin and Rom, Hassan},
  journal={arXiv preprint arXiv:2106.02443},
  year={2021}
}


@article{daram2020exploring,
  title={Exploring neuromodulation for dynamic learning},
  author={Daram, Anurag and Yanguas-Gil, Angel and Kudithipudi, Dhireesha},
  journal={Frontiers in Neuroscience},
  volume={14},
  pages={928},
  year={2020},
  publisher={Frontiers Media SA}
}


@article{lungu2020siamese,
  title={Siamese networks for few-shot learning on edge embedded devices},
  author={Lungu, Iulia Alexandra and Aimar, Alessandro and Hu, Yuhuang and Delbruck, Tobi and Liu, Shih-Chii},
  journal={IEEE Journal on Emerging and Selected Topics in Circuits and Systems},
  volume={10},
  number={4},
  pages={488--497},
  year={2020},
  publisher={IEEE}
}


@inproceedings{jiang2021few,
  title={Pseudo-loss confidence metric for semi-supervised few-shot learning},
  author={Huang, Kai and Geng, Jie and Jiang, Wen and Deng, Xinyang and Xu, Zhe},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={8671--8680},
  year={2021}
}


@article{imam2020rapid,
  title={Rapid online learning and robust recall in a neuromorphic olfactory circuit},
  author={Imam, Nabil and Cleland, Thomas A},
  journal={Nature Machine Intelligence},
  volume={2},
  number={3},
  pages={181--191},
  year={2020},
  publisher={Nature Publishing Group UK London}
}


@article{stewart2020online,
  title={Online few-shot gesture learning on a neuromorphic processor},
  author={Stewart, Kenneth and Orchard, Garrick and Shrestha, Sumit Bam and Neftci, Emre},
  journal={IEEE Journal on Emerging and Selected Topics in Circuits and Systems},
  volume={10},
  number={4},
  pages={512--521},
  year={2020},
  publisher={IEEE}
}



@article{van2019three,
  title={Three scenarios for continual learning},
  author={Van de Ven, Gido M and Tolias, Andreas S},
  journal={arXiv preprint arXiv:1904.07734},
  year={2019}
}

@inproceedings{scholar,
  title={SCOLAR: A Spiking Digital Accelerator with Dual Fixed Point for Continual Learning},
  author={Karia, Vedant and Zohora, Fatima Tuz and Soures, Nicholas and Kudithipudi, Dhireesha},
  booktitle={2022 IEEE International Symposium on Circuits and Systems (ISCAS)},
  pages={1372--1376},
  year={2022},
  organization={IEEE}
}


@article{neftci2018data,
  title={Data and power efficient intelligence with neuromorphic learning machines},
  author={Neftci, Emre O},
  journal={Iscience},
  volume={5},
  pages={52--68},
  year={2018},
  publisher={Elsevier}
}


@inproceedings{chen2014small,
  title={Small-footprint keyword spotting using deep neural networks},
  author={Chen, Guoguo and Parada, Carolina and Heigold, Georg},
  booktitle={2014 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={4087--4091},
  year={2014},
  organization={IEEE}
}

@article{berg2021keyword,
  title={Keyword transformer: A self-attention model for keyword spotting},
  author={Berg, Axel and O'Connor, Mark and Cruz, Miguel Tairum},
  journal={arXiv preprint arXiv:2104.00769},
  year={2021}
}


@inproceedings{sun2016max,
  title={Max-pooling loss training of long short-term memory networks for small-footprint keyword spotting},
  author={Sun, Ming and Raju, Anirudh and Tucker, George and Panchapagesan, Sankaran and Fu, Gengshen and Mandal, Arindam and Matsoukas, Spyros and Strom, Nikko and Vitaladevuni, Shiv},
  booktitle={2016 IEEE Spoken Language Technology Workshop (SLT)},
  pages={474--480},
  year={2016},
  organization={IEEE}
}


@article{arik2017convolutional,
  title={Convolutional recurrent neural networks for small-footprint keyword spotting},
  author={Arik, Sercan O and Kliegl, Markus and Child, Rewon and Hestness, Joel and Gibiansky, Andrew and Fougner, Chris and Prenger, Ryan and Coates, Adam},
  journal={arXiv preprint arXiv:1703.05390},
  year={2017}
}


@article{seo2021wav2kws,
  title={Wav2kws: Transfer learning from speech representations for keyword spotting},
  author={Seo, Deokjin and Oh, Heung-Seon and Jung, Yuchul},
  journal={IEEE Access},
  volume={9},
  pages={80682--80691},
  year={2021},
  publisher={IEEE}
}


@inproceedings{yilmaz2020deep,
  title={Deep convolutional spiking neural networks for keyword spotting},
  author={Y{\i}lmaz, Emre and Gevrek, Ozg{\"u}r Bora and Wu, Jibin and Chen, Yuxiang and Meng, Xuanbo and Li, Haizhou},
  booktitle={Proceedings of INTERSPEECH},
  pages={2557--2561},
  year={2020}
}



@inproceedings{blouw2019benchmarking,
  title={Benchmarking keyword spotting efficiency on neuromorphic hardware},
  author={Blouw, Peter and Choo, Xuan and Hunsberger, Eric and Eliasmith, Chris},
  booktitle={Proceedings of the 7th annual neuro-inspired computational elements workshop},
  pages={1--8},
  year={2019}
}

@article{chundi2021always,
  title={Always-on sub-microwatt spiking neural network based on spike-driven clock-and power-gating for an ultra-low-power intelligent device},
  author={Chundi, Pavan Kumar and Wang, Dewei and Kim, Sung Justin and Yang, Minhao and Cerqueira, Joao Pedro and Kang, Joonsung and Jung, Seungchul and Kim, Sangjoon and Seok, Mingoo},
  journal={Frontiers in Neuroscience},
  volume={15},
  pages={684113},
  year={2021},
  publisher={Frontiers Media SA}
}

@inproceedings{Krizhevsky2009LearningML,
  title={Learning Multiple Layers of Features from Tiny Images},
  author={Alex Krizhevsky},
  year={2009}
}

@misc{orchard2015converting,
      title={Converting Static Image Datasets to Spiking Neuromorphic Datasets Using Saccades}, 
      author={Garrick Orchard and Ajinkya Jayawant and Gregory Cohen and Nitish Thakor},
      year={2015},
      eprint={1507.07629},
      archivePrefix={arXiv},
      primaryClass={cs.DB}
}

@article{Cramer_2022,
	doi = {10.1109/tnnls.2020.3044364},
  
	url = {https://doi.org/10.1109%2Ftnnls.2020.3044364},
  
	year = 2022,
	month = {jul},
  
	publisher = {Institute of Electrical and Electronics Engineers ({IEEE})},
  
	volume = {33},
  
	number = {7},
  
	pages = {2744--2757},
  
	author = {Benjamin Cramer and Yannik Stradmann and Johannes Schemmel and Friedemann Zenke},
  
	title = {The Heidelberg Spiking Data Sets for the Systematic Evaluation of Spiking Neural Networks},
  
	journal = {{IEEE} Transactions on Neural Networks and Learning Systems}
}



  @article{guo2020neural,
  title={Neural network accelerator comparison},
  author={Guo, Kaiyuan and Li, Wenshuo and Zhong, Kai and Zhu, Z and Zeng, S and Han, S and Xie, Y and Debacker, P and Verhelst, M and Wang, Y},
  journal={NICS Lab of Tsinghua University. http://nicsefc. ee. tsinghua. edu. cn/projects/neural-network-accelerator},
  year={2020}
}

@article{rueckauer2022nxtf,
  title={NxTF: An API and compiler for deep spiking neural networks on Intel Loihi},
  author={Rueckauer, Bodo and Bybee, Connor and Goettsche, Ralf and Singh, Yashwardhan and Mishra, Joyesh and Wild, Andreas},
  journal={ACM Journal on Emerging Technologies in Computing Systems (JETC)},
  volume={18},
  number={3},
  pages={1--22},
  year={2022},
  publisher={ACM New York, NY}
}


@misc{lava,
    title={Lava Software Framework},
    author={Intel},
    year={2021},
howpublished = {\url{https://github.com/lava-nc/lava}}}

@misc{schuman2017survey,
      title={A Survey of Neuromorphic Computing and Neural Networks in Hardware}, 
      author={Catherine D. Schuman and Thomas E. Potok and Robert M. Patton and J. Douglas Birdwell and Mark E. Dean and Garrett S. Rose and James S. Plank},
      year={2017},
      eprint={1705.06963},
      archivePrefix={arXiv},
      primaryClass={cs.NE}
}

@article{james17historical,
title = {A historical survey of algorithms and hardware architectures for neural-inspired and neuromorphic computing applications},
author = {James, Conrad D. and Aimone, James B. and Miner, Nadine E. and Vineyard, Craig M. and Rothganger, Fredrick H. and Carlson, Kristofor D. and Mulder, Samuel A. and Draelos, Timothy J. and Faust, Aleksandra and Marinella, Matthew J. and Naegle, John H. and Plimpton, Steven J.},
abstractNote = {In this study, biological neural networks continue to inspire new developments in algorithms and microelectronic hardware to solve challenging data processing and classification problems. Here in this research, we survey the history of neural-inspired and neuromorphic computing in order to examine the complex and intertwined trajectories of the mathematical theory and hardware developed in this field. Early research focused on adapting existing hardware to emulate the pattern recognition capabilities of living organisms. Contributions from psychologists, mathematicians, engineers, neuroscientists, and other professions were crucial to maturing the field from narrowly-tailored demonstrations to more generalizable systems capable of addressing difficult problem classes such as object detection and speech recognition. Algorithms that leverage fundamental principles found in neuroscience such as hierarchical structure, temporal integration, and robustness to error have been developed, and some of these approaches are achieving world-leading performance on particular data classification tasks. Additionally, novel microelectronic hardware is being developed to perform logic and to serve as memory in neuromorphic computing systems with optimized system integration and improved energy efficiency. Key to such advancements was the incorporation of new discoveries in neuroscience research, the transition away from strict structural replication and towards the functional replication of neural systems, and the use of mathematical theory frameworks to guide algorithm and hardware developments.},
doi = {10.1016/j.bica.2016.11.002},
journal = {Biologically Inspired Cognitive Architectures},
volume = 19,
place = {United States},
year = {2017},
month = {1}
}

@misc{thakur2018largescale,
      title={Large-Scale Neuromorphic Spiking Array Processors: A quest to mimic the brain}, 
      author={Chetan Singh Thakur and Jamal Molin and Gert Cauwenberghs and Giacomo Indiveri and Kundan Kumar and Ning Qiao and Johannes Schemmel and Runchun Wang and Elisabetta Chicca and Jennifer Olson Hasler and Jae-sun Seo and Shimeng Yu and Yu Cao and André van Schaik and Ralph Etienne-Cummings},
      year={2018},
      eprint={1805.08932},
      archivePrefix={arXiv},
      primaryClass={cs.NE}
}

@article{deng2012mnist,
  title={The mnist database of handwritten digit images for machine learning research},
  author={Deng, Li},
  journal={IEEE Signal Processing Magazine},
  volume={29},
  number={6},
  pages={141--142},
  year={2012},
  publisher={IEEE}
}


@article{bretteandgerstner2005,
author = {Brette, Romain and Gerstner, Wulfram},
title = {Adaptive Exponential Integrate-and-Fire Model as an Effective Description of Neuronal Activity},
journal = {Journal of Neurophysiology},
volume = {94},
number = {5},
pages = {3637-3642},
year = {2005},
doi = {10.1152/jn.00686.2005},
    note ={PMID: 16014787},
}

@article{maass2000computational,
  title={On the computational power of winner-take-all},
  author={Maass, Wolfgang},
  journal={Neural computation},
  volume={12},
  number={11},
  pages={2519--2535},
  year={2000},
  publisher={MIT Press}
}

@article{auge2021survey,
  title={A survey of encoding techniques for signal processing in spiking neural networks},
  author={Auge, Daniel and Hille, Julian and Mueller, Etienne and Knoll, Alois},
  journal={Neural Processing Letters},
  volume={53},
  number={6},
  pages={4693--4710},
  year={2021},
  publisher={Springer}
}

@inproceedings{schemmel2010wafer,
  title={A wafer-scale neuromorphic hardware system for large-scale neural modeling},
  author={Schemmel, Johannes and Br{\"u}derle, Daniel and Gr{\"u}bl, Andreas and Hock, Matthias and Meier, Karlheinz and Millner, Sebastian},
  booktitle={2010 ieee international symposium on circuits and systems (iscas)},
  pages={1947--1950},
  year={2010},
  organization={IEEE}
}

@article{bouvier2019spiking,
  title={Spiking neural networks hardware implementations and challenges: A survey},
  author={Bouvier, Maxence and Valentian, Alexandre and Mesquida, Thomas and Rummens, Francois and Reyboz, Marina and Vianello, Elisa and Beigne, Edith},
  journal={ACM Journal on Emerging Technologies in Computing Systems (JETC)},
  volume={15},
  number={2},
  pages={1--35},
  year={2019},
  publisher={ACM New York, NY, USA}
}

@misc{van2021neural,
  title={Neural processor based accelerator system and method},
  author={van der Made, Peter AJ and Mankar, Anil Shamrao},
  year={2021},
  month=oct # "~26",
  publisher={Google Patents},
  note={US Patent 11,157,800}
}

@misc{synsensespeck,
  title = {Speck},
  howpublished = {\url{https://www.synsense.ai/products/speck/}},
  note = {Accessed: 2023-04-03}
}

@article{tang2017sparse,
  title={Sparse coding by spiking neural networks: Convergence theory and computational results},
  author={Tang, Ping Tak Peter and Lin, Tsung-Han and Davies, Mike},
  journal={arXiv preprint arXiv:1705.05475},
  year={2017}
}

@article{frolich2019gest,
author = {Fröhlich, Marlen and Sievers, Christine and Townsend, Simon W. and Gruber, Thibaud and van Schaik, Carel P.},
title = {Multimodal communication and language origins: integrating gestures and vocalizations},
journal = {Biological Reviews},
volume = {94},
number = {5},
pages = {1809-1829},
keywords = {evolution of language, cognition, ontogeny, gestural origins, vocal origins, primates, comparative approach, learning, multimodality},
doi = {10.1111/brv.12535},
url = {https://onlinelibrary.wiley.com/doi/abs/10.1111/brv.12535},
eprint = {https://onlinelibrary.wiley.com/doi/pdf/10.1111/brv.12535},
year = {2019}
}

@article{Young2020car,
   title={Designing Mid-Air Haptic Gesture Controlled User Interfaces for Cars},
   volume={4},
   ISSN={2573-0142},
   url={http://dx.doi.org/10.1145/3397869},
   DOI={10.1145/3397869},
   number={EICS},
   journal={Proceedings of the ACM on Human-Computer Interaction},
   publisher={Association for Computing Machinery (ACM)},
   author={Young, Gareth and Milne, Hamish and Griffiths, Daniel and Padfield, Elliot and Blenkinsopp, Robert and Georgiou, Orestis},
   year={2020},
   month={Jun},
   pages={1–23}
}

@inproceedings{may2017carlicit,
author = {May, Keenan R. and Gable, Thomas M. and Walker, Bruce N.},
title = {Designing an In-Vehicle Air Gesture Set Using Elicitation Methods},
year = {2017},
isbn = {9781450351508},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3122986.3123015},
doi = {10.1145/3122986.3123015},
booktitle = {Proceedings of the 9th International Conference on Automotive User Interfaces and Interactive Vehicular Applications},
pages = {74–83},
numpages = {10},
keywords = {Workload, Participatory Design, Gestures},
location = {Oldenburg, Germany},
series = {AutomotiveUI '17}
}

@inproceedings{balati2018dysarthric,
author = {Ballati, Fabio and Corno, Fulvio and De Russis, Luigi},
title = {Assessing Virtual Assistant Capabilities with Italian Dysarthric Speech},
year = {2018},
isbn = {9781450356503},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3234695.3236354},
doi = {10.1145/3234695.3236354},
booktitle = {Proceedings of the 20th International ACM SIGACCESS Conference on Computers and Accessibility},
pages = {93–101},
numpages = {9},
keywords = {speech impairment, automatic speech recognition, accessibility, conversational assistant, dysarthria},
location = {Galway, Ireland},
series = {ASSETS '18}
}


@misc{MLCommon79:online,
author = {},
title = {MLCommons},
howpublished = {\url{https://mlcommons.org/en/}},
month = {},
year = {},
note = {(Accessed on 04/04/2023)}
}

@ARTICLE{zhang2012kinect,  author={Z. {Zhang}},  journal={IEEE MultiMedia},   title={Microsoft Kinect Sensor and Its Effect},   year={2012},  volume={19},  number={2},  pages={4-10},}

@InProceedings{Keselman2017Realsense,
author = {Keselman, Leonid and Iselin Woodfill, John and Grunnet-Jepsen, Anders and Bhowmik, Achintya},
title = {Intel RealSense Stereoscopic Depth Cameras},
booktitle = {Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition (CVPR) Workshops},
month = {July},
year = {2017}
}

@inproceedings{wang2016soli, author = {Wang, Saiwen and Song, Jie and Lien, Jaime and Poupyrev, Ivan and Hilliges, Otmar}, title = {Interacting with Soli: Exploring Fine-Grained Dynamic Gesture Recognition in the Radio-Frequency Spectrum}, year = {2016}, isbn = {9781450341899}, publisher = {Association for Computing Machinery}, address = {New York, NY, USA}, url = {https://doi.org/10.1145/2984511.2984565}, doi = {10.1145/2984511.2984565}, booktitle = {Proceedings of the 29th Annual Symposium on User Interface Software and Technology}, pages = {851–860}, numpages = {10}, keywords = {wearables, gesture recognition, radar sensing, deep learning}, location = {Tokyo, Japan}, series = {UIST ’16} }

@Article{Lichtsteiner_etal08_128x120,
author		= {Lichtsteiner, P. and Posch, C. and Delbruck, T.},
doi		= {10.1109/JSSC.2007.914337},
issn		= {0018-9200},
journal		= {Solid-State Circuits, IEEE Journal of},
keyword		= {{CMOS} image sensors{CMOS} vision sensor, active
		  continuous-time front-end logarithmic photoreceptor,
		  address-event representation, bandwidth 3 kHz, chip power
		  consumption, image sensor, latency asynchronous temporal
		  contrast vision sensor, power 23 mW, self-timed
		  switched-capacitor differencing circuit, silicon retina,
		  size 0.35 um, spike event, time 15 us},
month		= {Feb.},
number		= {2},
pages		= {566--576},
title		= {A 128x128 120 {dB} 15 us Latency Asynchronous Temporal
		  Contrast Vision Sensor},
volume		= {43},
year		= {2008}
}

@Article{Hakim2019ic4you,
author={Hakim, Noorkholis Luthfil
and Shih, Timothy K.
and Kasthuri Arachchi, Sandeli Priyanwada
and Aditya, Wisnu
and Chen, Yi-Cheng
and Lin, Chih-Yang},
title={Dynamic Hand Gesture Recognition Using 3DCNN and LSTM with FSM Context-Aware Model},
journal={Sensors (Basel, Switzerland)},
year={2019},
month={Dec},
day={09},
publisher={MDPI},
volume={19},
number={24},
pages={5429},
keywords={context-aware; deep learning; hand gesture recognition; multimodal system},
note={31835404[pmid]},
issn={1424-8220},
doi={10.3390/s19245429},
url={https://pubmed.ncbi.nlm.nih.gov/31835404},
url={https://doi.org/10.3390/s19245429},
language={eng}
}

@InProceedings{Amir_etal17_lowpowe,
author		= {Amir, Arnon and Taba, Brian and Berg, David and Melano,
		  Timothy and McKinstry, Jeffrey and Di Nolfo, Carmelo and
		  Nayak, Tapan and Andreopoulos, Alexander and Garreau,
		  Guillaume and Mendoza, Marcela and others},
booktitle	= {Proceedings of the IEEE Conference on Computer Vision and
		  Pattern Recognition},
pages		= {7243--7252},
title		= {A Low Power, Fully Event-Based Gesture Recognition
		  System},
year		= {2017}
}

@Article{Mead90_neurelec,
author		= {C. Mead},
journal		= {Proceedings of the {IEEE}},
keyword		= {neuromorphic avlsi system},
number		= {10},
pages		= {1629--36},
title		= {Neuromorphic Electronic Systems},
volume		= {78},
year		= {1990}
}

@Article{Indiveri_etal11_neursili,
author		= {G. Indiveri and B. Linares-Barranco and T.J. Hamilton and
		  A. van Schaik and R. Etienne-Cummings and T. Delbruck and
		  S.-C. Liu and P. Dudek and P. H{\"a}fliger and S. Renaud
		  and J. Schemmel and G. Cauwenberghs and J. Arthur and K.
		  Hynna and F. Folowosele and S. Saighi and T.
		  Serrano-Gotarredona and J. Wijekoon and Y. Wang and K.
		  Boahen},
doi		= {10.3389/fnins.2011.00073},
issn		= {1662-453X},
journal		= {Frontiers in Neuroscience},
link		= {http://www.frontiersin.org/Neuromorphic_Engineering/10.3389/fnins.2011.00073/abstract},
pages		= {1--23},
title		= {Neuromorphic silicon neuron circuits},
volume		= {5},
year		= {2011}
}

@Article{Davies19_bencprog,
title		= {Benchmarks for progress in neuromorphic computing},
author		= {Davies, Mike},
journal		= {Nature Machine Intelligence},
volume		= {1},
number		= {9},
pages		= {386388},
year		= {2019},
publisher	= {Nature Publishing Group}
}

@Article{Chicca_etal13_neurelec,
author		= {Chicca, E. and Stefanini, F. and Indiveri, G.},
journal		= {Proceedings of {IEEE}},
title		= {Neuromorphic electronic circuits for building autonomous
		  cognitive systems},
year		= {2013}
}

@Article{Pfeil_etal12_4bitsyna,
author		= {T. Pfeil and T. C. Potjans and S. Schrader and W. Potjans
		  and J. Schemmel and M. Diesmann and K. Meier},
doi		= {10.3389/fnins.2012.00090},
issn		= {1662453X},
journal		= {Frontiers in Neuroscience},
link		= {http://www.frontiersin.org/Journal/Abstract.aspx?s=755&name=neuromorphic_engineering&ART_DOI=10.3389/fnins.2012.00090},
title		= {Is a 4bit synaptic weight resolution enough?  Constraints
		  on enabling spiketiming dependent plasticity in
		  neuromorphic hardware},
volume		= {6},
year		= {2012}
}



@Article{Neftci18_datapowe,
title		= {Data and Power Efficient Intelligence with Neuromorphic
		  Learning Machines},
journal		= {iScience},
volume		= {5},
month		= {jul},
pages		= {5268},
year		= {2018},
issn		= {25890042},
doi		= {https://doi.org/10.1016/j.isci.2018.06.010},
author		= {Emre O. Neftci},
keywords	= {Systems Neuroscience, Computer Science, Evolvable
		  Hardware},
url		= {https://www.sciencedirect.com/science/article/pii/S2589004218300865}
}

@inproceedings{zhuang2016unrestricted,
  author={Yimeng Zhuang and Xuankai Chang and Yanmin Qian and Kai Yu},
  title={{Unrestricted Vocabulary Keyword Spotting Using LSTM-CTC}},
  year=2016,
  booktitle={Proc. Interspeech 2016},
  pages={938--942},
  doi={10.21437/Interspeech.2016-753}
}

@article{hoy2018alexa,
author = {Hoy, Matthew},
year = {2018},
month = {01},
pages = {81-88},
title = {Alexa, Siri, Cortana, and More: An Introduction to Voice Assistants},
volume = {37},
journal = {Medical Reference Services Quarterly},
doi = {10.1080/02763869.2018.1404391}
}

@INPROCEEDINGS{michaely2017keyword,
  author={Michaely, Assaf Hurwitz and Zhang, Xuedong and Simko, Gabor and Parada, Carolina and Aleksic, Petar},
  booktitle={2017 IEEE Automatic Speech Recognition and Understanding Workshop (ASRU)}, 
  title={Keyword spotting for Google assistant using contextual speech recognition}, 
  year={2017},
  volume={},
  number={},
  pages={272-278},
  doi={10.1109/ASRU.2017.8268946}}

  @article{kitayama2022guiding,
  title={Guiding principle of reservoir computing based on “small-world” network},
  author={Kitayama, Ken-ichi},
  journal={Scientific reports},
  volume={12},
  number={1},
  pages={16697},
  year={2022},
  publisher={Nature Publishing Group UK London}
}

@article{hilgetag2016brain,
  title={Is the brain really a small-world network?},
  author={Hilgetag, Claus C and Goulas, Alexandros},
  journal={Brain Structure and Function},
  volume={221},
  pages={2361--2366},
  year={2016},
  publisher={Springer}
}

@inproceedings{schuman2019non,
  title={Non-traditional input encoding schemes for spiking neuromorphic systems},
  author={Schuman, Catherine D and Plank, James S and Bruer, Grant and Anantharaj, Jeremy},
  booktitle={2019 International Joint Conference on Neural Networks (IJCNN)},
  pages={1--10},
  year={2019},
  organization={IEEE}
}

@inproceedings{schuman2020evolutionary,
  title={Evolutionary optimization for neuromorphic systems},
  author={Schuman, Catherine D and Mitchell, J Parker and Patton, Robert M and Potok, Thomas E and Plank, James S},
  booktitle={Proceedings of the Neuro-inspired Computational Elements Workshop},
  pages={1--9},
  year={2020}
}

@inproceedings{shrestha2017stable,
  title={Stable spike-timing dependent plasticity rule for multilayer unsupervised and supervised learning},
  author={Shrestha, Amar and Ahmed, Khadeer and Wang, Yanzhi and Qiu, Qinru},
  booktitle={2017 international joint conference on neural networks (IJCNN)},
  pages={1999--2006},
  year={2017},
  organization={IEEE}
}

@article{tanaka2019recent,
  title={Recent advances in physical reservoir computing: A review},
  author={Tanaka, Gouhei and Yamane, Toshiyuki and H{\'e}roux, Jean Benoit and Nakane, Ryosho and Kanazawa, Naoki and Takeda, Seiji and Numata, Hidetoshi and Nakano, Daiju and Hirose, Akira},
  journal={Neural Networks},
  volume={115},
  pages={100--123},
  year={2019},
  publisher={Elsevier}
}

@article{hunsberger2016training,
  title={Training spiking deep networks for neuromorphic hardware},
  author={Hunsberger, Eric and Eliasmith, Chris},
  journal={arXiv preprint arXiv:1611.05141},
  year={2016}
}

@inproceedings{alemi2018learning,
  title={Learning nonlinear dynamics in efficient, balanced spiking networks using local plasticity rules},
  author={Alemi, Alireza and Machens, Christian and Deneve, Sophie and Slotine, Jean-Jacques},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={32},
  number={1},
  year={2018}
}

@article{wunderlich2019demonstrating,
  title={Demonstrating advantages of neuromorphic computation: a pilot study},
  author={Wunderlich, Timo and Kungl, Akos F and M{\"u}ller, Eric and Hartel, Andreas and Stradmann, Yannik and Aamir, Syed Ahmed and Gr{\"u}bl, Andreas and Heimbrecht, Arthur and Schreiber, Korbinian and St{\"o}ckel, David and others},
  journal={Frontiers in neuroscience},
  volume={13},
  pages={260},
  year={2019},
  publisher={Frontiers Media SA}
}

@article{furber2016large,
  title={Large-scale neuromorphic computing systems},
  author={Furber, Steve},
  journal={Journal of neural engineering},
  volume={13},
  number={5},
  pages={051001},
  year={2016},
  publisher={IOP Publishing}
}


@misc{tidigits, note={R. Gary Leonard, and George Doddington. TIDIGITS LDC93S10. Web Download. Philadelphia: Linguistic Data Consortium, 1993.}}

@article{frenkel2021bottom,
  title={Bottom-up and top-down neural processing systems design: Neuromorphic intelligence as the convergence of natural and artificial intelligence},
  author={Frenkel, Charlotte and Bol, David and Indiveri, Giacomo},
  journal={arXiv preprint arXiv:2106.01288},
  year={2021}
}
@article{azghadi2014spike,
  title={Spike-based synaptic plasticity in silicon: design, implementation, application, and challenges},
  author={Azghadi, Mostafa Rahimi and Iannella, Nicolangelo and Al-Sarawi, Said F and Indiveri, Giacomo and Abbott, Derek},
  journal={Proceedings of the IEEE},
  volume={102},
  number={5},
  pages={717--737},
  year={2014},
  publisher={IEEE}
}

@article{zenke2021brain,
  title={Brain-inspired learning on neuromorphic substrates},
  author={Zenke, Friedemann and Neftci, Emre O},
  journal={Proceedings of the IEEE},
  volume={109},
  number={5},
  pages={935--950},
  year={2021},
  publisher={IEEE}
}

@article{mysore2022hierarchical,
  title={Hierarchical network connectivity and partitioning for reconfigurable large-scale neuromorphic systems},
  author={Mysore, Nishant and Hota, Gopabandhu and Deiss, Stephen R and Pedroni, Bruno U and Cauwenberghs, Gert},
  journal={Frontiers in Neuroscience},
  volume={15},
  pages={1891},
  year={2022},
  publisher={Frontiers}
}

@article{Dalgaty2023,
doi = {10.21203/rs.3.rs-2651639/v1},
url = {https://doi.org/10.21203/rs.3.rs-2651639/v1},
year = {2023},
month = mar,
publisher = {Research Square Platform {LLC}},
author = {Thomas Dalgaty and Filippo Moro and Yi{\u{g}}it Demira{\u{g}} and Alessio De Pra and Giacomo Indiveri and Elisa Vianello and Melika Payvand},
title = {The neuromorphic Mosaic: in-memory computing and routing for small-world graphical networks}
}

@article{indiveri2015memory,
  title={Memory and information processing in neuromorphic systems},
  author={Indiveri, Giacomo and Liu, Shih-Chii},
  journal={Proceedings of the IEEE},
  volume={103},
  number={8},
  pages={1379--1397},
  year={2015},
  publisher={IEEE}
}

@article{frenkel20180,
  title={A 0.086-mm $\^{} 2 $12.7-pJ/SOP 64k-synapse 256-neuron online-learning digital spiking neuromorphic processor in 28-nm CMOS},
  author={Frenkel, Charlotte and Lefebvre, Martin and Legat, Jean-Didier and Bol, David},
  journal={IEEE transactions on biomedical circuits and systems},
  volume={13},
  number={1},
  pages={145--158},
  year={2018},
  publisher={IEEE}
}

@inproceedings{frenkel202028,
  title={A 28-nm convolutional neuromorphic processor enabling online learning with spike-based retinas},
  author={Frenkel, Charlotte and Legat, Jean-Didier and Bol, David},
  booktitle={2020 IEEE International Symposium on Circuits and Systems (ISCAS)},
  pages={1--5},
  year={2020},
  organization={IEEE}
}

@inproceedings{seo201145nm,
  title={A 45nm CMOS neuromorphic chip with a scalable architecture for learning in networks of spiking neurons},
  author={Seo, Jae-sun and Brezzo, Bernard and Liu, Yong and Parker, Benjamin D and Esser, Steven K and Montoye, Robert K and Rajendran, Bipin and Tierno, Jos{\'e} A and Chang, Leland and Modha, Dharmendra S and others},
  booktitle={2011 IEEE Custom Integrated Circuits Conference (CICC)},
  pages={1--4},
  year={2011},
  organization={IEEE}
}

@article{park201965,
  title={A 65-nm neuromorphic image classification processor with energy-efficient training through direct spike-only feedback},
  author={Park, Jeongwoo and Lee, Juyun and Jeon, Dongsuk},
  journal={IEEE Journal of Solid-State Circuits},
  volume={55},
  number={1},
  pages={108--119},
  year={2019},
  publisher={IEEE}
}

@article{chen20184096,
  title={A 4096-neuron 1M-synapse 3.8-pJ/SOP spiking neural network with on-chip STDP learning and sparse weights in 10-nm FinFET CMOS},
  author={Chen, Gregory K and Kumar, Raghavan and Sumbul, H Ekin and Knag, Phil C and Krishnamurthy, Ram K},
  journal={IEEE Journal of Solid-State Circuits},
  volume={54},
  number={4},
  pages={992--1002},
  year={2018},
  publisher={IEEE}
}

@article{knag2015sparse,
  title={A sparse coding neural network ASIC with on-chip learning for feature extraction and encoding},
  author={Knag, Phil and Kim, Jung Kuk and Chen, Thomas and Zhang, Zhengya},
  journal={IEEE Journal of Solid-State Circuits},
  volume={50},
  number={4},
  pages={1070--1079},
  year={2015},
  publisher={IEEE}
}

@article{frenkel2019morphic,
  title={MorphIC: A 65-nm 738k-Synapse/mm \^{} 2 quad-core binary-weight digital neuromorphic processor with stochastic spike-driven online learning},
  author={Frenkel, Charlotte and Legat, Jean-Didier and Bol, David},
  journal={IEEE transactions on biomedical circuits and systems},
  volume={13},
  number={5},
  pages={999--1010},
  year={2019},
  publisher={IEEE}
}

@inproceedings{cassidy2013cognitive,
  title={Cognitive computing building block: A versatile and efficient digital neuron model for neurosynaptic cores},
  author={Cassidy, Andrew S and Merolla, Paul and Arthur, John V and Esser, Steve K and Jackson, Bryan and Alvarez-Icaza, Rodrigo and Datta, Pallab and Sawada, Jun and Wong, Theodore M and Feldman, Vitaly and others},
  booktitle={The 2013 International Joint Conference on Neural Networks (IJCNN)},
  pages={1--10},
  year={2013},
  organization={IEEE}
}

@article{Sanni:2019bv,
author = {Sanni, Kayode A and Andreou, Andreas G},
title = {{A Historical Perspective on Hardware AI Inference, Charge-Based Computational Circuits and an 8bit Charge-Based Multiply-Add Core in {16nm FinFET CMOS}}},
journal = {IEEE Journal on Emerging and Selected Topics in Circuits and Systems},
year = {2019},
volume = {9},
number = {3},
pages = {532--543},
month = sep,
affiliation = {Johns Hopkins University, Baltimore, United States},
doi = {10.1109/JETCAS.2019.2933795},
}

@inproceedings{moreira2020neuronflow,
title={NeuronFlow: a neuromorphic processor architecture for live AI applications},
author={Moreira, Orlando and Yousefzadeh, Amirreza and Chersi, Fabian and Cinserin, Gokturk and Zwartenkot, Rik-Jan and Kapoor, Ajay and Qiao, Peng and Kievits, Peter and Khoei, Mina and Rouillard, Louis and others},
booktitle={2020 Design, Automation \& Test in Europe Conference \& Exhibition (DATE)},
pages={840--845},
year={2020},
organization={IEEE}
}

@article{lillicrap2020backpropagation,
  title={Backpropagation and the brain},
  author={Lillicrap, Timothy P and Santoro, Adam and Marris, Luke and Akerman, Colin J and Hinton, Geoffrey},
  journal={Nature Reviews Neuroscience},
  volume={21},
  number={6},
  pages={335--346},
  year={2020},
  publisher={Nature Publishing Group UK London}
}

@article{neftci2019surrogate,
  title={Surrogate gradient learning in spiking neural networks: Bringing the power of gradient-based optimization to spiking neural networks},
  author={Neftci, Emre O and Mostafa, Hesham and Zenke, Friedemann},
  journal={IEEE Signal Processing Magazine},
  volume={36},
  number={6},
  pages={51--63},
  year={2019},
  publisher={IEEE}
}

@inproceedings{bohnstingl2022biologically,
  title={Biologically-inspired training of spiking recurrent neural networks with neuromorphic hardware},
  author={Bohnstingl, Thomas and {\v{S}}urina, Anja and Fabre, Maxime and Demira{\u{g}}, Yi{\u{g}}it and Frenkel, Charlotte and Payvand, Melika and Indiveri, Giacomo and Pantazi, Angeliki},
  booktitle={2022 IEEE 4th International Conference on Artificial Intelligence Circuits and Systems (AICAS)},
  pages={218--221},
  year={2022},
  organization={IEEE}
}

@article{izhikevich2004model,
  title={Which model to use for cortical spiking neurons?},
  author={Izhikevich, Eugene M},
  journal={IEEE transactions on neural networks},
  volume={15},
  number={5},
  pages={1063--1070},
  year={2004},
  publisher={Ieee}
}

@article{mannion2023artificial,
  title={Artificial Dendritic Computation: The case for dendrites in neuromorphic circuits},
  author={Mannion, Daniel John and Kenyon, Anthony John},
  journal={arXiv preprint arXiv:2304.00951},
  year={2023}
}

@article{sangwan2020neuromorphic,
  title={Neuromorphic nanoelectronic materials},
  author={Sangwan, Vinod K and Hersam, Mark C},
  journal={Nature nanotechnology},
  volume={15},
  number={7},
  pages={517--528},
  year={2020},
  publisher={Nature Publishing Group UK London}
}

@InProceedings{chi2022metafscil,
    author    = {Chi, Zhixiang and Gu, Li and Liu, Huan and Wang, Yang and Yu, Yuanhao and Tang, Jin},
    title     = {MetaFSCIL: A Meta-Learning Approach for Few-Shot Class Incremental Learning},
    booktitle = {Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
    month     = {June},
    year      = {2022},
    pages     = {14166-14175}
}

@misc{stewart2022metalearning,
    title={Meta-learning Spiking Neural Networks with Surrogate Gradient Descent},
    author={Kenneth Stewart and Emre Neftci},
    year={2022},
    eprint={2201.10777},
    archivePrefix={arXiv},
    primaryClass={cs.NE}
}

@INPROCEEDINGS{liao2022ethsnn,
  author={Liao, Jiawei and Widmer, Lars and Wang, Xiaying and Di Mauro, Alfio and Nason-Tomaszewski, Samuel R. and Chestek, Cynthia A. and Benini, Luca and Jang, Taekwang},
  booktitle={2022 IEEE 4th International Conference on Artificial Intelligence Circuits and Systems (AICAS)}, 
  title={An Energy-Efficient Spiking Neural Network for Finger Velocity Decoding for Implantable Brain-Machine Interface}, 
  year={2022},
  volume={},
  number={},
  pages={134-137},
  doi={10.1109/AICAS54282.2022.9869846}}

@article{shahi2022prediction,
title = {Prediction of chaotic time series using recurrent neural networks and reservoir computing techniques: A comparative study},
journal = {Machine Learning with Applications},
volume = {8},
pages = {100300},
year = {2022},
issn = {2666-8270},
doi = {https://doi.org/10.1016/j.mlwa.2022.100300},
url = {https://www.sciencedirect.com/science/article/pii/S2666827022000275},
author = {Shahrokh Shahi and Flavio H. Fenton and Elizabeth M. Cherry},
keywords = {Recurrent neural networks, Reservoir computing, Echo state networks, Deep learning, Chaotic time series, Nonlinear vector autoregression},
abstract = {In recent years, machine-learning techniques, particularly deep learning, have outperformed traditional time-series forecasting approaches in many contexts, including univariate and multivariate predictions. This study aims to investigate the capability of (i) gated recurrent neural networks, including long short-term memory (LSTM) and gated recurrent unit (GRU) networks, (ii) reservoir computing (RC) techniques, such as echo state networks (ESNs) and hybrid physics-informed ESNs, and (iii) the nonlinear vector autoregression (NVAR) approach, which has recently been introduced as the next generation RC, for the prediction of chaotic time series and to compare their performance in terms of accuracy, efficiency, and robustness. We apply the methods to predict time series obtained from two widely used chaotic benchmarks, the Mackey–Glass and Lorenz-63 models, as well as two other chaotic datasets representing a bursting neuron and the dynamics of the El Niño Southern Oscillation, and to one experimental dataset representing a time series of cardiac voltage with complex dynamics. We find that even though gated RNN techniques have been successful in forecasting time series generally, they can fall short in predicting chaotic time series for the methods, datasets, and ranges of hyperparameter values considered here. In contrast, for the chaotic datasets studied, we found that reservoir computing and NVAR techniques are more computationally efficient and offer more promise in long-term prediction of chaotic time series.}
}

@misc{top500,
title={TOP500},
    author={TOP500},
    year={2023},
howpublished = {\url{https://www.top500.org/}}}

@misc{green500,
title={Green500},
    author={Green500},
    year={2023},
howpublished = {\url{https://www.top500.org/lists/green500/}}
}

@misc{mlperfpower,
title={MLCommons Power Working Group},
    author={MLCommons},
    year={2023},
howpublished = {\url{https://mlcommons.org/en/groups/best-practices-power/}}
}

@misc{gilpin2023largescale,
      title={Large-scale statistical forecasting models reassess the unpredictability of chaotic systems}, 
      author={William Gilpin},
      year={2023},
      eprint={2303.08011},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@misc{dai2016deep,
      title={Very Deep Convolutional Neural Networks for Raw Waveforms}, 
      author={Wei Dai and Chia Dai and Shuhui Qu and Juncheng Li and Samarjit Das},
      year={2016},
      eprint={1610.00087},
      archivePrefix={arXiv},
      primaryClass={cs.SD}
}

@article{Aimone2022,

doi = {10.1088/2634-4386/ac889c},

url = {https://dx.doi.org/10.1088/2634-4386/ac889c},

year = {2022},

month = {sep},

publisher = {IOP Publishing},

volume = {2},

number = {3},

pages = {032003},

author = {James B Aimone and Prasanna Date and Gabriel A Fonseca-Guerra and Kathleen E Hamilton and Kyle Henke and Bill Kay and Garrett T Kenyon and Shruti R Kulkarni and Susan M Mniszewski and Maryam Parsa and Sumedh R Risbud and Catherine D Schuman and William Severa and J Darby Smith},

title = {A review of non-cognitive applications for neuromorphic computing},

journal = {Neuromorphic Computing and Engineering },

}


@misc{mlperf_policies,
    title={MLPerf Inference Policies},
    author={MLCommons},
    year={2023},
howpublished = {\url{https://github.com/mlcommons/inference_policies/}}}

@ARTICLE{spynnaker,
  
AUTHOR={Rhodes, Oliver and Bogdan, Petruţ A. and Brenninkmeijer, Christian and Davidson, Simon and Fellows, Donal and Gait, Andrew and Lester, David R. and Mikaitis, Mantas and Plana, Luis A. and Rowley, Andrew G. D. and Stokes, Alan B. and Furber, Steve B.},   
	 
TITLE={sPyNNaker: A Software Package for Running PyNN Simulations on SpiNNaker},      
	
JOURNAL={Frontiers in Neuroscience},      
	
VOLUME={12},           
	
YEAR={2018},      
	  
URL={https://www.frontiersin.org/articles/10.3389/fnins.2018.00816},       
	
DOI={10.3389/fnins.2018.00816},      
	
ISSN={1662-453X},   
   
ABSTRACT={This work presents sPyNNaker 4.0.0, the latest version of the software package for simulating PyNN-defined spiking neural networks (SNNs) on the SpiNNaker neuromorphic platform. Operations underpinning realtime SNN execution are presented, including an event-based operating system facilitating efficient time-driven neuron state updates and pipelined event-driven spike processing. Preprocessing, realtime execution, and neuron/synapse model implementations are discussed, all in the context of a simple example SNN. Simulation results are demonstrated, together with performance profiling providing insights into how software interacts with the underlying hardware to achieve realtime execution. System performance is shown to be within a factor of 2 of the original design target of 10,000 synaptic events per millisecond, however SNN topology is shown to influence performance considerably. A cost model is therefore developed characterizing the effect of network connectivity and SNN partitioning. This model enables users to estimate SNN simulation performance, allows the SpiNNaker team to make predictions on the impact of performance improvements, and helps demonstrate the continued potential of the SpiNNaker neuromorphic hardware.}
}

@misc{nir2023,
  author       = {Abreu, Steven and
                  Bauer, Felix and
                  Eshraghian, Jason and
                  Jobst, Matthias and
                  Lenz, Gregor and
                  Pedersen, Jens Egholm and
                  Sheik, Sadique},
  title        = {Neuromorphic Intermediate Representation},
  month        = jul,
  year         = 2023,
  publisher    = {Zenodo},
  version      = {0.0.1},
  doi          = {10.5281/zenodo.8105042},
  url          = {https://doi.org/10.5281/zenodo.8105042}
}

@article{taillard1993,

title = {Benchmarks for basic scheduling problems},

journal = {European Journal of Operational Research},

volume = {64},

number = {2},

pages = {278-285},

year = {1993},

note = {Project Management anf Scheduling},

issn = {0377-2217},

doi = {https://doi.org/10.1016/0377-2217(93)90182-M},

url = {https://www.sciencedirect.com/science/article/pii/037722179390182M},

author = {E. Taillard},

}

@article{koch2022,

title = {Progress in mathematical programming solvers from 2001 to 2020},

journal = {EURO Journal on Computational Optimization},

volume = {10},

pages = {100031},

year = {2022},

issn = {2192-4406},

doi = {https://doi.org/10.1016/j.ejco.2022.100031},

url = {https://www.sciencedirect.com/science/article/pii/S2192440622000077},

author = {Thorsten Koch and Timo Berthold and Jaap Pedersen and Charlie Vanaret},

}

@article{fra22har,
author = {Fra, Vittorio and Forno, Evelina and Pignari, Riccardo and Stewart, Terrence and Macii, Enrico and Urgese, Gianvito},
year = {2022},
month = {01},
pages = {},
title = {Human activity recognition: suitability of a neuromorphic approach for on-edge AIoT applications},
volume = {2},
journal = {Neuromorphic Computing and Engineering},
doi = {10.1088/2634-4386/ac4c38}
}

@inproceedings{pellegrini20latent,
  author={Pellegrini, Lorenzo and Graffieti, Gabriele and Lomonaco, Vincenzo and Maltoni, Davide},
  booktitle={2020 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)}, 
  title={Latent Replay for Real-Time Continual Learning}, 
  year={2020},
  volume={},
  number={},
  pages={10203-10209},
  doi={10.1109/IROS45743.2020.9341460}}


@Article{ScardapaneRandomness2017,
	title = {Randomness in Neural Networks: an Overview},
	author = {Scardapane, Simone and Wang, Dianhui},
	journal = "{Data Mining and Knowledge Discovery}",
	year = {2017},
	volume = {7},
	number = {2},
	pages = {1--18},
    doi={10.1002/widm.1200}
}

@ARTICLE{bittar22surrogate,
  
AUTHOR={Bittar, Alexandre and Garner, Philip N.},   
	 
TITLE={A surrogate gradient spiking baseline for speech command recognition},      
	
JOURNAL={Frontiers in Neuroscience},      
	
VOLUME={16},           
	
YEAR={2022},      
	  
URL={https://www.frontiersin.org/articles/10.3389/fnins.2022.865897},       
	
DOI={10.3389/fnins.2022.865897},      
	
ISSN={1662-453X},   
   
ABSTRACT={Artificial neural networks (ANNs) are the basis of recent advances in artificial intelligence (AI); they typically use real valued neuron responses. By contrast, biological neurons are known to operate using spike trains. In principle, spiking neural networks (SNNs) may have a greater representational capability than ANNs, especially for time series such as speech; however their adoption has been held back by both a lack of stable training algorithms and a lack of compatible baselines. We begin with a fairly thorough review of literature around the conjunction of ANNs and SNNs. Focusing on surrogate gradient approaches, we proceed to define a simple but relevant evaluation based on recent speech command tasks. After evaluating a representative selection of architectures, we show that a combination of adaptation, recurrence and surrogate gradients can yield light spiking architectures that are not only able to compete with ANN solutions, but also retain a high degree of compatibility with them in modern deep learning frameworks. We conclude tangibly that SNNs are appropriate for future research in AI, in particular for speech processing applications, and more speculatively that they may also assist in inference about biological function.}
}

@inproceedings{stewart23speech2spikes,
author = {Stewart, Kenneth Michael and Shea, Timothy and Pacik-Nelson, Noah and Gallo, Eric and Danielescu, Andreea},
title = {Speech2Spikes: Efficient Audio Encoding Pipeline for Real-Time Neuromorphic Systems},
year = {2023},
isbn = {9781450399470},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3584954.3584995},
doi = {10.1145/3584954.3584995},
abstract = {Despite the maturity and availability of speech recognition systems, there are few available spiking speech recognition tasks that can be implemented with current neuromorphic systems. The methods used previously to generate spiking speech data are not capable of encoding speech in real-time or encoding very large modern speech datasets efficiently for input to neuromorphic processors. The ability to efficiently encode audio data to spikes will enable a wider variety of spiking audio datasets to be available and can also enable algorithmic development of real-time neuromorphic automatic speech recognition systems. Therefore, we developed speech2spikes, a simple and efficient audio processing pipeline that encodes recorded audio into spikes and is suitable for real-time operation with low-power neuromorphic processors. To demonstrate the efficacy of our method for audio to spike encoding we show that a small feed-forward spiking neural network trained on data generated with the pipeline achieves accuracy on the Google Speech Commands recognition task, exceeding the state-of-the art set by Spiking Speech Commands, a prior spiking encoding of the Google Speech Commands dataset, by over 10\%. We also demonstrate a proof-of-concept real-time neuromorphic automatic speech recognition system using audio encoded with speech2spikes streamed to an Intel Loihi neuromorphic research processor.},
booktitle = {Proceedings of the 2023 Annual Neuro-Inspired Computational Elements Conference},
pages = {71–78},
numpages = {8},
keywords = {Neuromorphic Computing, Spike Encoding, Speech Recognition, Spiking Neural Networks},
location = {San Antonio, TX, USA},
series = {NICE '23}
}

@ARTICLE{frenkel23bottom,
  author={Frenkel, Charlotte and Bol, David and Indiveri, Giacomo},
  journal={Proceedings of the IEEE}, 
  title={Bottom-Up and Top-Down Approaches for the Design of Neuromorphic Processing Systems: Tradeoffs and Synergies Between Natural and Artificial Intelligence}, 
  year={2023},
  volume={111},
  number={6},
  pages={623-652},
  doi={10.1109/JPROC.2023.3273520}}

@article{Hochreiter1997,
  doi = {10.1162/neco.1997.9.8.1735},
  url = {https://doi.org/10.1162/neco.1997.9.8.1735},
  year = {1997},
  publisher = {{MIT} Press - Journals},
  volume = {9},
  number = {8},
  pages = {1735--1780},
  author = {Sepp Hochreiter and J\"{u}rgen Schmidhuber},
  title = {Long Short-Term Memory},
  journal = {Neural Computation}
}

@inproceedings{
jeffares2022spikeinspired,
title={Spike-inspired rank coding for fast and accurate recurrent neural networks},
author={Alan Jeffares and Qinghai Guo and Pontus Stenetorp and Timoleon Moraitis},
booktitle={International Conference on Learning Representations},
year={2022},
url={https://openreview.net/forum?id=iMH1e5k7n3L}
}

@article{Johansson2004FirstSI,
  title={First spikes in ensembles of human tactile afferents code complex spatial fingertip events},
  author={Roland S. Johansson and Ingvars Birznieks},
  journal={Nature Neuroscience},
  year={2004},
  volume={7},
  pages={170-177},
  url={https://api.semanticscholar.org/CorpusID:1182173}
}

@article{jitcxde,
	author = {Gerrit Ansmann},
	title = {Efficiently and easily integrating differential equations with {JiTCODE}, {JiTCDDE}, and {JiTCSDE}},
	year = {2018},
	journal = {Chaos},
	volume = {28},
	number = {4},
	pages = {043116},
	doi = {10.1063/1.5019320},
}


@misc{metavision,
    title={Event-Based Vision Software - Metavision Intelligence},
    author={Prophesee},
    year={2023},
howpublished = {\url{https://www.prophesee.ai/metavision-intelligence/}}}


@article{MAKRIDAKIS202054,
title = {The M4 Competition: 100,000 time series and 61 forecasting methods},
journal = {International Journal of Forecasting},
volume = {36},
number = {1},
pages = {54-74},
year = {2020},
note = {M4 Competition},
issn = {0169-2070},
doi = {https://doi.org/10.1016/j.ijforecast.2019.04.014},
url = {https://www.sciencedirect.com/science/article/pii/S0169207019301128},
author = {Spyros Makridakis and Evangelos Spiliotis and Vassilios Assimakopoulos},
keywords = {Forecasting competitions, M competitions, Forecasting accuracy, Prediction intervals, Time series methods, Machine learning methods, Benchmarking methods, Practice of forecasting},
abstract = {The M4 Competition follows on from the three previous M competitions, the purpose of which was to learn from empirical evidence both how to improve the forecasting accuracy and how such learning could be used to advance the theory and practice of forecasting. The aim of M4 was to replicate and extend the three previous competitions by: (a) significantly increasing the number of series, (b) expanding the number of forecasting methods, and (c) including prediction intervals in the evaluation process as well as point forecasts. This paper covers all aspects of M4 in detail, including its organization and running, the presentation of its results, the top-performing methods overall and by categories, its major findings and their implications, and the computational requirements of the various methods. Finally, it summarizes its main conclusions and states the expectation that its series will become a testing ground for the evaluation of new methods and the improvement of the practice of forecasting, while also suggesting some ways forward for the field.}
}

@incollection{Lemaire_2023,
	doi = {10.1007/978-3-031-30105-6_48},
  
	url = {https://doi.org/10.1007%2F978-3-031-30105-6_48},
  
	year = 2023,
	publisher = {Springer International Publishing},
  
	pages = {574--587},
  
	author = {Edgar Lemaire and Loïc Cordone and Andrea Castagnetti and Pierre-Emmanuel Novac and Jonathan Courtois and Beno{\^{\i}
}t Miramond},
  
	title = {An Analytical Estimation of~Spiking Neural Networks Energy Efficiency},
  
	booktitle = {Neural Information Processing}
}

@article{kudithipudi22biological,
author = {Kudithipudi, Dhireesha and Aguilar-Simon, Mario and Babb, Jonathan and Bazhenov, Maxim and Blackiston, Douglas and Bongard, Josh and Brna, Andrew and Chakravarthi Raja, Suraj and Cheney, Nick and Clune, Jeff and Daram, Anurag and Fusi, Stefano and Helfer, Peter and Kay, Leslie and Ketz, Nicholas and Kira, Zsolt and Kolouri, Soheil and Krichmar, Jeff and Kriegman, Sam and Siegelmann, Hava},
year = {2022},
month = {03},
pages = {196-210},
title = {Biological underpinnings for lifelong learning machines},
volume = {4},
journal = {Nature Machine Intelligence},
doi = {10.1038/s42256-022-00452-0}
}

@INPROCEEDINGS{hu18squeeze,
  author={Hu, Jie and Shen, Li and Sun, Gang},
  booktitle={2018 IEEE/CVF Conference on Computer Vision and Pattern Recognition}, 
  title={Squeeze-and-Excitation Networks}, 
  year={2018},
  volume={},
  number={},
  pages={7132-7141},
  doi={10.1109/CVPR.2018.00745}}

@inproceedings{shi15convlstm,
author = {Shi, Xingjian and Chen, Zhourong and Wang, Hao and Yeung, Dit-Yan and Wong, Wai-kin and Woo, Wang-chun},
title = {Convolutional LSTM Network: A Machine Learning Approach for Precipitation Nowcasting},
year = {2015},
publisher = {MIT Press},
address = {Cambridge, MA, USA},
abstract = {The goal of precipitation nowcasting is to predict the future rainfall intensity in a local region over a relatively short period of time. Very few previous studies have examined this crucial and challenging weather forecasting problem from the machine learning perspective. In this paper, we formulate precipitation nowcasting as a spatiotemporal sequence forecasting problem in which both the input and the prediction target are spatiotemporal sequences. By extending the fully connected LSTM (FC-LSTM) to have convolutional structures in both the input-to-state and state-to-state transitions, we propose the convolutional LSTM (ConvLSTM) and use it to build an end-to-end trainable model for the precipitation nowcasting problem. Experiments show that our ConvLSTM network captures spatiotemporal correlations better and consistently outperforms FC-LSTM and the state-of-the-art operational ROVER algorithm for precipitation nowcasting.},
booktitle = {Proceedings of the 28th International Conference on Neural Information Processing Systems - Volume 1},
pages = {802–810},
numpages = {9},
location = {Montreal, Canada},
series = {NIPS'15}
}

@incollection{Liu_2016,
	doi = {10.1007/978-3-319-46448-0_2},
  
	url = {https://doi.org/10.1007%2F978-3-319-46448-0_2},
  
	year = 2016,
	publisher = {Springer International Publishing},
  
	pages = {21--37},
  
	author = {Wei Liu and Dragomir Anguelov and Dumitru Erhan and Christian Szegedy and Scott Reed and Cheng-Yang Fu and Alexander C. Berg},
  
	title = {{SSD}: Single Shot {MultiBox} Detector},
  
	booktitle = {Computer Vision {\textendash} {ECCV} 2016}
}

@INPROCEEDINGS{sevilla22computetrends,
  author={Sevilla, Jaime and Heim, Lennart and Ho, Anson and Besiroglu, Tamay and Hobbhahn, Marius and Villalobos, Pablo},
  booktitle={2022 International Joint Conference on Neural Networks (IJCNN)}, 
  title={Compute Trends Across Three Eras of Machine Learning}, 
  year={2022},
  volume={},
  number={},
  pages={1-8},
  doi={10.1109/IJCNN55064.2022.9891914}}

@INPROCEEDINGS{shankar22trends,
  author={Shankar, Sadasivan and Reuther, Albert},
  booktitle={2022 IEEE High Performance Extreme Computing Conference (HPEC)}, 
  title={Trends in Energy Estimates for Computing in AI/Machine Learning Accelerators, Supercomputers, and Compute-Intensive Applications}, 
  year={2022},
  volume={},
  number={},
  pages={1-8},
  doi={10.1109/HPEC55821.2022.9926296}}

@article{ray22tinyml,
title = {A review on TinyML: State-of-the-art and prospects},
journal = {Journal of King Saud University - Computer and Information Sciences},
volume = {34},
number = {4},
pages = {1595-1623},
year = {2022},
issn = {1319-1578},
doi = {https://doi.org/10.1016/j.jksuci.2021.11.019},
url = {https://www.sciencedirect.com/science/article/pii/S1319157821003335},
author = {Partha Pratim Ray},
keywords = {TinyML, IoT, Edge intelligence, Energy efficient AI, Resource constrained intelligence, Embedded AI},
abstract = {Machine learning has become an indispensable part of the existing technological domain. Edge computing and Internet of Things (IoT) together presents a new opportunity to imply machine learning techniques at the resource constrained embedded devices at the edge of the network. Conventional machine learning requires enormous amount of power to predict a scenario. Embedded machine learning – TinyML paradigm aims to shift such plethora from traditional high-end systems to low-end clients. Several challenges are paved while doing such transition such as, maintaining the accuracy of learning models, provide train-to-deploy facility in resource frugal tiny edge devices, optimizing processing capacity, and improving reliability. In this paper, we present an intuitive review about such possibilities for TinyML. We firstly, present background of TinyML. Secondly, we list the tool sets for supporting TinyML. Thirdly, we present key enablers for improvement of TinyML systems. Fourthly, we present state-of-the-art about frameworks for TinyML. Finally, we identify key challenges and prescribe a future roadmap for mitigating several research issues of TinyML.}
}

@article{willsey22realtime,
author = {Willsey, Matthew and Nason-Tomaszewski, Samuel and Ensel, Scott and Temmar, Hisham and Mender, Matthew and Costello, Joseph and Patil, Parag and Chestek, Cynthia},
year = {2022},
month = {11},
pages = {6899},
title = {Real-time brain-machine interface in non-human primates achieves high-velocity prosthetic finger movements using a shallow feedforward neural network decoder},
volume = {13},
journal = {Nature Communications},
doi = {10.1038/s41467-022-34452-w}
}
